CREPE: Can Vision-Language Foundation Models Reason Compositionally?

A fundamental characteristic common to both human vision and natural language is their compositional nature. Yet, despite the performance gains contributed by large vision and language pretraining, we find that: across 7 architectures trained with 4 algorithms on massive datasets, they struggle at compositionality. To arrive at this conclusion, we introduce a new compositionality evaluation benchmark, CREPE, which measures two important aspects of compositionality identified by cognitive science literature: systematicity and productivity. To measure systematicity, CREPE consists of a test dataset containing over $370K$ image-text pairs and three different seen-unseen splits. The three splits are designed to test models trained on three popular training datasets: CC-12M, YFCC-15M, and LAION-400M. We also generate $325K$, $316K$, and $309K$ hard negative captions for a subset of the pairs. To test productivity, CREPE contains $17K$ image-text pairs with nine different complexities plus $183K$ hard negative captions with atomic, swapping and negation foils. The datasets are generated by repurposing the Visual Genome scene graphs and region descriptions and applying handcrafted templates and GPT-3. For systematicity, we find that model performance decreases consistently when novel compositions dominate the retrieval set, with Recall@1 dropping by up to $12\%$. For productivity, models' retrieval success decays as complexity increases, frequently nearing random chance at high complexity. These results hold regardless of model and training dataset size.

==> figures/modelPerfvsRecall_prod.tex <==
\begin{figure}[t!]
     \centering
     \includegraphics[width=.95\columnwidth]{figures/prodHN.pdf}
     \caption{\textit{Productivity Analysis}. We plot the retrieval Recall@1 of all models trained on all three datasets. We observe that there is no consistent correlation with model size within datasets.}
     \label{fig:prodModelPerf}
 \end{figure}

==> figures/modelPerfvsRecall_syst.tex <==
\begin{figure}[t!]
     \centering
     \includegraphics[width=0.95\columnwidth]{figures/systHN.pdf}
     \caption{\textit{Systematicity Analysis.} We plot the retrieval Recall@1 of all models pretrained on the three datasets and observe no particular correlation with model size within datasets.}
     \label{fig:systModelPerf}
 \end{figure}

==> figures/syst_hn_atom_recall_at_avg_k.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/syst_hn_atom_avg recall@k_plot.pdf}
    \caption{A plot showing the difference between modes' average recall@k (k=1,3) on the Seen Compounds and Unseen Compounds splits of the systematicity \textsc{HN-Atom} sets.}
    \label{fig:syst_hn_atom_recall_at_avg_k}
\end{figure}

==> figures/syst_hn_combined_recall_at_1.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/syst_hn_combined_recall@1_plot.pdf}
    \caption{A plot showing the difference between modes' recall@1 on the Seen Compounds and Unseen Compounds splits of the systematicity \textbf{\textsc{HN-Atom} + \textsc{HN-Comp}} combined sets.}
    \label{fig:syst_hn_combined_recall_at_1}
\end{figure}

==> old/00_abstract_v1.tex <==
Vision-language models have recently demonstrated great success across various visual linguistic tasks such as image captioning, visual question answering etc. In particular, models trained with the Contrastive Language–Image Pre-training objective (CLIP models) have shown competitive performance in diverse downstream tasks. The success of CLIP has inspired the development of different CLIP model variants for a wide range of applications from object detection to image synthesis. 
Despite inumerable adaptations and applications of CLIP, only a few works try to understand the properties of the image and text representations learned by CLIP models and why they are useful or not. One crucial property of learned representations is compositionality, which is also tied to a model's generalizability and interpretability.
In this paper, we develop a benchmark CLIPComp for evaluating the compositionality of CLIP models' representations via retrieval. We focus on two important aspects of compositionality - systematicity and productivity, and we establish procedures and release datasets to evaluate pretrained CLIP models' systematicity and productivity.
% Our systematicity evaluation method is applicable to all pretrained CLIP models with known training dataset, and our procedure for productivity evaluation is universally applicable. 
We repurpose the Visual Genome scene graphs as our evaluation dataset and augment it with image captions generated with handcrafted templates and GPT3. Our evaluation dataset contains x, y, z image-text pairs for systematicity evaluation of CLIP models pretrained on CC12M, YFCC15M, and Laion400M as well as 20K groundtruth captions and 200K negatives for productivity evaluation.  
We find that while pretrained CLIP models have reasonable zero-shot performance on both image-to-text and text-to-image retrieval, their performances decrease by  x\% on average as novel compositions dominate the retrieval set. They also suffer from a significant performance drop as the complexity of the texts increases. 
These results suggest that CLIP models struggle at both systematicity and productivity. Our benchmark provides insights into CLIP models' failure modes through an evaluation of the compositionality of their representations and encourages future work to build more compositional vision-language models. 


% State of the world: CLIP experiences great success. Various applications. Gives rise to related approaches inspired by it.


% What's missing/why is this hard: Given the prevalence of CLIP and influx of new approaches, we need to better evaluate and understand these models. A proper statement of why finetuning performance and existing zero-shot evaluation is insufficient.

% Bit-flip: We provide an evaluation pipeline focused on compositionality allowing researchers to assess what the representations trained by the pretraining methods contain. Systematicity. Different from past work: productivity and a dataset independent replicable evaluation pipeline. Details on evaluation. Details on dataset size on both tasks.

% Results: How do models perform. What surprising insights do we get. Implications for future work.



==> old/00_abstract_v2.tex <==
Vision-language models have recently demonstrated great success across various visual-linguistic tasks such as image captioning, visual question answering etc. In particular, models trained with the Contrastive Language–Image Pre-training objective (CLIP models) have shown competitive performance in diverse downstream tasks. The success of CLIP has inspired the development of different CLIP model variants for a wide range of applications from object detection to image synthesis. 
Despite inumerable adaptations and applications of CLIP, only a few works try to understand the properties of the image and text representations learned by CLIP models and why they are useful or not. One crucial property of learned representations is compositionality, which is also tied to a model's generalizability and interpretability.
In this paper, we develop a benchmark CLIPComp for evaluating the compositionality of CLIP models' representations via retrieval. We focus on two important aspects of compositionality - systematicity and productivity, and we establish procedures and release datasets to evaluate pretrained CLIP models' systematicity and productivity.
% Our systematicity evaluation method is applicable to all pretrained CLIP models with known training dataset, and our procedure for productivity evaluation is universally applicable. 
We repurpose the Visual Genome scene graphs as our evaluation dataset and augment it with image captions generated with handcrafted templates and GPT3. Our evaluation dataset contains x, y, z image-text pairs for systematicity evaluation of CLIP models pretrained on CC12M, YFCC15M, and Laion400M as well as 20K groundtruth captions and 200K negatives for productivity evaluation.  
We find that while pretrained CLIP models have reasonable zero-shot performance on both image-to-text and text-to-image retrieval, their performances decrease by  x\% on average as novel compositions dominate the retrieval set. They also suffer from a significant performance drop as the complexity of the texts increases. 
These results suggest that CLIP models struggle at both systematicity and productivity. Our benchmark provides insights into CLIP models' failure modes through an evaluation of the compositionality of their representations and encourages future work to build more compositional vision-language models. 


% State of the world: CLIP experiences great success. Various applications. Gives rise to related approaches inspired by it.


% What's missing/why is this hard: Given the prevalence of CLIP and influx of new approaches, we need to better evaluate and understand these models. A proper statement of why finetuning performance and existing zero-shot evaluation is insufficient.

% Bit-flip: We provide an evaluation pipeline focused on compositionality allowing researchers to assess what the representations trained by the pretraining methods contain. Systematicity. Different from past work: productivity and a dataset independent replicable evaluation pipeline. Details on evaluation. Details on dataset size on both tasks.

% Results: How do models perform. What surprising insights do we get. Implications for future work.



==> old/00_abstract_v3.tex <==


% Sentences that need to be in the abstract:
% 1. establish that compositionality is important for vision and for language.
% 2. mention that we don't know if existing models exhibit compositionality.
% 3. Say that we introduce a benchmark (needs a name) that evaluated whether models exhibit two kinds of compositionality: systematicity and productivity.
% 4. One sentence about how the dataset was built and what the size of the dataset is.
% 5. One sentence about which models were evaluated using this benchmark
% 6. One sentence about the main takeaway.
% 7. Final sentence about implications: why do these results matter and how does it inform us.
A fundamental characteristic common to both human vision and natural language is their compositional nature. Yet, despite the ubiquitous performance gains contributed by large vision and language pretraining, we find that the resulting models exhibit little compositionality.
To arrive at this conclusion, we introduce a new compositionality evaluation benchmark—\nameemoji{}—which measures two important aspects of compositionality identified by cognitive science literature: systematicity and productivity. To measure systematicity, \name{} consists of three test datasets. The three test sets are designed to test models trained on three of the popular training datasets: CC-12M, YFCC-15M, and LAION-400M. They contain $385K$, $385K$ and $373K$ image-text pairs and $237K$, $210K$ and $178K$ hard negative captions. To test productivity, \name{} contains $17K$ image-text pairs with nine different complexities plus $246K$ hard negative captions with atomic, swapping and negation foils. The datasets are generated by repurposing the Visual Genome scene graphs and region descriptions and applying handcrafted templates and GPT3.
For systematicity, we find that model performance decreases consistently when novel compositions dominate the retrieval set, with Recall@1 dropping by up to $8\%$. For productivity, models' retrieval success decays as complexity increases, nearing random chance at high complexity. These results hold regardless of model and training dataset size. 

==> old/01_introduction_v0.tex <==
Like NLP, vision-language research has recently undergone a paradigm shift away from specialized architectures for particular tasks and towards large, self-supervised models pre-trained on large quantities of data adapted to downstream tasks. Such applications which are based upon these large vision-language models, such as CLIP and ALIGN, continue to grow in breadth and sophistication. However, our understanding of these models remains poor; in particular, we have yet to fully assess their \textit{compositional} capabilities.

In human language and reasoning, compositionality lends us a remarkable capacity to understand complex visual scenes and sentences by building them up from simple atomic parts. \textit{On top of that, compositionality addresses (reword?)} the impossible task of memorizing each possible sentence or visual scene by allowing us to systematically generalize to unseen stimuli. It is therefore natural that compositionality in vision-language models is not only a vital indicator of reasoning capability but also a desirable property for a variety of applications, from disentangling complex environments in robotic settings to handling granular edits in controllable image generation. \textit{TODO: connect these specifically to the shared visuosemantic representation space}

% What's missing:
    % While we have indirect confirmation that these models are capable of some forms of compositionality, such as the impressive ability of DALL-E 2 to combine disparate concepts into coherent scenes, there is a dearth of probing tasks directly investigating whether the learned representations allow for compositionality.
        % Counter-argument: What's wrong with finetuning? Couldn't you perform a linear probe, for instance, on GQA? That should be informative. Why can we also not apply any of the existing linear probes developed for BERT?
            % Answer 1: These models can be used directly as a loss function/evaluation metric without further finetuning. This is why we care about the particular representation space. 
            % Response: Still, linear probing experiments \textit{can} give feedback on what information these representations contain. 
            % Answer 2: Perhaps motivate things from the zero-shot perspective. Why should anyone care about the exact representations?
            % Answer 3: What kinds of confounders do linear probing experiments introduce? The model can pick up on dataset/language biases, for one. I'm sure that there are criticisms of the linear probing set up in both recent vision evaluation work and in the NLP literature.
    % Claim (that needs evidence): Existing benchmarks that allow for zero-shot generalization, such as image classification or retrieval datasets, cannot be used to stress-test compositionality in a directed manner.

Currently, we lack a rigorous, direct evaluation of the compositional capabilities of large vision-language models. Recent architectures which rely on (frozen?) vision-language representations, such as DALL-E 2, hint at promising vision-language compositional capabilities. However, these are at best indirect indicators of the compositionality of said representations. Other downstream applications analyze CLIP's zero-shot performance on tasks such as image captioning or retrieval. These provide direct insights on what information its representations hold, but they fail to stress-test compositionality.

% Why this is hard:
    % 

% Bit-flip:
    % We propose a new retrieval benchmark built from VG scene graph annotations that can be used to probe whether the visuo-semantic representation spaces of large pre-trained models allow for compositional reasoning.
    % Our benchmark has two splits for two facets of compositionality: systematicity and productivity. 
    % Why retrieval? 1) Similarity scores are hard to interpret, rank ordering is more interpretable with a carefully designed dataset. 2) Visually evaluating generated images adds a confounding factor (generator) and...human subjectivity?
        % Counterpoint: who is even claiming that raw similarity scores would be a good benchmark?
    % [TODO] We focus on representations; reiterate why.
    
To allow for direct evaluations of whether these models' shared visuosemantic representation spaces allow for compositionality, we propose a retrieval benchmark built from the scene graph annotations within Visual Genome. Our benchmark probes for two crucial and orthogonal aspects of compositionality. The first is \textit{systematicity}, which captures how well a model can generalizes to unseen compositions of concepts. The second is \textit{productivity}, which captures how well a model can process complex scenes and scene descriptions. Both compositionality tests require the retrieval dataset to encompass an exhaustive combination of attributes, objects, and relationships; we therefore introduce a set of augmentations which ensure that, for any Visual Genome data point, there exist sufficiently similar images and captions that a model with weaker compositionality would confound with said data point. \textit{More detail about this augmentation?} In contrast to evaluation with generated images and linear probes, which introduce confounding architectures, relying on retrieval from this novel dataset allows us to truly probe the compositionality of the representation space.

% TODO: results
% How can these findings generalize to 5 years from now?
% a framework for assessing compositionality in multimodal models
% a new image2text & text2image retrieval dataset

==> old/01_introduction_v2.tex <==
\section{Introduction}

% A fundamental characteristic common to both human vision and natural language is their compositional nature. People can communicate and imagine a scene of a "biker in an orange jacket riding a bike.


% State of the world:
    % Introduce compositionality and how V+L tasks benefit from it
    % Remark upon the popularity and success of large pre-trained models in V+L. Standard set-up: Either finetune representations from these models on downstream tasks or leverage the representations in a zero-shot manner.
        % Not sure about how to scope this part. Do we only care about models trained with a contrastive loss like CLIP or broaden the horizon to include older pretrained models like LXMERT as well?
    % As these models more commonly become the basis of V+L applications, it is crucial that they represent the necessary information for compositional reasoning.
        % Another difficult part. "Necessary information for compositional reasoning" feels hand-wavy. At the same time, the representations themselves are not compositional. The terminology needs to be more precise.
        
%[Jerry] Here's a proposed transition from V&L models to composition: Vision and language's new "foundation model" paradigm -> these models are growing in popularity -> these models remain poorly understood, specifically in compositionality. Human thought/reasoning is compositional, and this is what it allows; likewise, here's why it's useful in vision-language. [Omer] I think this flows more naturally but let's see
% [Jerry] Would we be interested in discussing compositionality as "the wall", the benchmark that models seemed to have been unable to reach? This is a strong claim requiring strong evidence. [Omer] Nah, I think motivating why compositionality is important is more helpful.

In recent years, vision-language research has been experiencing a shift away from crafting specialized architectures for particular tasks towards the design of task-agnostic models pre-trained with self-supervision on large datasets~(\cite{tan2019lxmert, lu2019vilbert, Zhang_2021_CVPR, Desai_2021_CVPR}). Among these models, CLIP~\cite{radford2021learning}, which learns a shared embedding space for images and text through a contrastive loss, has recently experienced great popularity, with promising use cases beyond standard fine-tuning on downstream tasks, such as zero-shot transfer~\cite{subramanian2022reclip} and automatic caption evaluation~\cite{hessel-etal-2021-clipscore}. As CLIP's applications increase, it becomes more important to understand and evaluate its capabilities.
        
One crucial capability for vision-language tasks is \textit{compositionality}, the ability to understand ``the meaning of a whole [a]s a function of the meanings of its parts''~\cite{cresswell1973logics}. For language, these parts are words while for visual scenes, they are the objects that populate scenes and their attributes, relationships and actions~\cite{krishnavisualgenome, ji2020action}. This capability is hypothesized to partly enable humans' ability to systematically generalize to novel, unseen inputs and can additionally confer beneficial properties such as interpretability or controllability to machine learning models~\cite{lake_ullman_tenenbaum_gershman_2017, bommasani2021opportunities}. Given compositionality's advantages, it is desirable for researchers to quantify whether CLIP's representations encode necessary information for compositional reasoning.


% What's missing:
    % While we have indirect confirmation that these models are capable of some forms of compositionality, such as the impressive ability of DALL-E 2 to combine disparate concepts into coherent scenes, there is a dearth of probing tasks directly investigating whether the learned representations allow for compositionality.
        % Counter-argument: What's wrong with finetuning? Couldn't you perform a linear probe, for instance, on GQA? That should be informative. Why can we also not apply any of the existing linear probes developed for BERT?
            % Answer 1: These models can be used directly as a loss function/evaluation metric without further finetuning. This is why we care about the particular representation space. 
            % Response: Still, linear probing experiments \textit{can} give feedback on what information these representations contain. 
            % Answer 2: Perhaps motivate things from the zero-shot perspective. Why should anyone care about the exact representations?
            % Answer 3: What kinds of confounders do linear probing experiments introduce? The model can pick up on dataset/language biases, for one. I'm sure that there are criticisms of the linear probing set up in both recent vision evaluation work and in the NLP literature.
    % Claim (that needs evidence): Existing benchmarks that allow for zero-shot generalization, such as image classification or retrieval datasets, cannot be used to stress-test compositionality in a directed manner.

Currently, our insights regarding whether CLIP encodes information for compositionality comes from indirect sources. For instance, while DALL-E 2~\citep{ramesh2022hierarchical}, which uses frozen CLIP text embeddings as its basis, can impressively compose distinct objects, scenes and attributes to generate coherent images, the complexity of its architecture makes it difficult to attribute its success to CLIP representations~\citep{hewitt-liang-2019-designing}. On the other hand, although studies that investigate CLIP's zero-shot performance~\citep{subramanian2022reclip} give direct insights into whether its representations are useful, they fail to stress-test compositionality.


% Bit-flip:
    % We propose a new retrieval benchmark built from VG scene graph annotations that can be used to probe whether the visuo-semantic representation spaces of large pre-trained models allow for compositional reasoning.
    % Our benchmark has two splits for two facets of compositionality: systematicity and productivity. 
    % Why retrieval? 1) Similarity scores are hard to interpret, rank ordering is more interpretable with a carefully designed dataset. 2) Visually evaluating generated images adds a confounding factor (generator) and...human subjectivity?
        % Counterpoint: who is even claiming that raw similarity scores would be a good benchmark?
    % [TODO] We focus on representations; reiterate why.
    
In this paper, we propose a retrieval benchmark built from scene graph annotations within Visual Genome~\citep{krishnavisualgenome} to allow for a direct evaluation of whether CLIP's representation space allows for compositionality. Our benchmark probes for two crucial and orthogonal aspects of compositionality. The first is \textit{systematicity}, which captures how well a model can generalizes to unseen compositions of concepts. The second is \textit{productivity}, which captures how well a model can process complex scenes and scene descriptions. Both compositionality tests require the retrieval dataset to encompass an exhaustive combination of attributes, objects, and relationships; we therefore introduce a set of augmentations which ensure that, for any Visual Genome data point, there exist sufficiently similar images and captions that a model with weaker compositionality would confound with said data point. \textit{More detail about this augmentation?} In contrast to evaluation with generated images and linear probes, which introduce confounding architectures, relying on retrieval from this novel dataset allows us to truly probe the compositionality of the representation space.

% TODO: results
% How can these findings generalize to 5 years from now?
% a framework for assessing compositionality in multimodal models
% a new image2text & text2image retrieval dataset

==> old/01_introduction_v3.tex <==
\section{Introduction}

% A fundamental characteristic common to both human vision and natural language is their compositional nature. People can communicate and imagine a scene of a "biker in an orange jacket riding a bike.


% State of the world:
    % Introduce compositionality and how V+L tasks benefit from it
    % Remark upon the popularity and success of large pre-trained models in V+L. Standard set-up: Either finetune representations from these models on downstream tasks or leverage the representations in a zero-shot manner.
        % Not sure about how to scope this part. Do we only care about models trained with a contrastive loss like CLIP or broaden the horizon to include older pretrained models like LXMERT as well?
    % As these models more commonly become the basis of V+L applications, it is crucial that they represent the necessary information for compositional reasoning.
        % Another difficult part. "Necessary information for compositional reasoning" feels hand-wavy. At the same time, the representations themselves are not compositional. The terminology needs to be more precise.
        
%[Jerry] Here's a proposed transition from V&L models to composition: Vision and language's new "foundation model" paradigm -> these models are growing in popularity -> these models remain poorly understood, specifically in compositionality. Human thought/reasoning is compositional, and this is what it allows; likewise, here's why it's useful in vision-language. [Omer] I think this flows more naturally but let's see
% [Jerry] Would we be interested in discussing compositionality as "the wall", the benchmark that models seemed to have been unable to reach? This is a strong claim requiring strong evidence. [Omer] Nah, I think motivating why compositionality is important is more helpful.

Comparative psychology, specifically Morgan's Canon~\cite{morgan1894introduction}, has come to appreciate that human researchers are vulnerable to systematic biases when comparing human and nonhuman intelligence. Understood as an error, Morgan's Canon is the tendency of people to attribute human-like capabilities to non-humans on the basis of insufficient empirical evidence. In an effort to avoid this error in interpreting the emergent machine capabilities~\cite{buckner2019comparative}, this paper focuses on evaluating today's popular vision-language foundation models. Given our learned models' propensity for shortcut learning~\cite{geirhos2020shortcut}, wherein they maximize benchmark performance while failing to generalize to real applications, it is vital that we uncover deficiencies in model behavior. Understanding model behavior is particularly vital for foundation models~\cite{radford2021learning}, which have ubiquitously become the ``foundation'' atop which other models are trained~\cite{conwell2022testing,ramesh2022hierarchical,saharia2022photorealistic}.

% In recent years, vision-language research has been experiencing a shift away from crafting specialized architectures for particular tasks towards the design of task-agnostic models pre-trained with self-supervision on large datasets~(\cite{tan2019lxmert, lu2019vilbert, Zhang_2021_CVPR, Desai_2021_CVPR}). Among these models, CLIP~\cite{radford2021learning}, which learns a shared embedding space for images and text through a contrastive loss, has recently experienced great popularity, with promising use cases beyond standard fine-tuning on downstream tasks, such as zero-shot transfer~\cite{subramanian2022reclip} and automatic caption evaluation~\cite{hessel-etal-2021-clipscore}. As CLIP's applications increase, it becomes more important to understand and evaluate its capabilities.
        
One crucial capability we expect to see in vision-language models is \textit{compositionality}, a fundamental human capability using which people understand new scenes and generate complex sentences~\cite{janssen1997compositionality,hupkes2020compositionality,bottou2014machine}. Compositionality allows us to understand ``the meaning of a whole [a]s a function of the meanings of its [atoms]''~\cite{cresswell1973logics}. For language, these atoms are words that form the sentence while for visual scenes, they are the objects that populate scenes along their attributes, relationships and actions~\cite{krishnavisualgenome,ji2020action}. Compositionality allows people to differentiate between ``TODO'' and ``TODO'' (Figure~\ref{fig:pull_figure}). This capability is hypothesized to partly enable humans' ability to systematically generalize to novel, unseen inputs and can additionally confer beneficial properties such as interpretability or controllability to machine learning models~\cite{lake_ullman_tenenbaum_gershman_2017,bommasani2021opportunities}. 
% Given compositionality's advantages, we investigate whether today's best vision-language models encode necessary information for compositional reasoning.

% We need a paragraph here about why it is hard to measure compositionality today.
While we have indirect confirmation that these models are capable of some forms of compositionality, such as the impressive ability of DALL-E 2 to combine disparate concepts into coherent scenes~\cite{ramesh2022hierarchical}, there is a dearth of probing evaluations directly investigating whether the learned representations allow for compositionality.
These models are trained using web-scraped datasets, comprised of millions of images with their associated text captions~\cite{thomee2016yfcc100m,schuhmann2021laion,sharma2018conceptual} 
%The dominant training paradigm is a contrastive objective~\cite{radford2021learning}; 
and evaluated using image-text retrieval~\cite{jia2021scaling,radford2021learning,Zhang_2021_CVPR}. Although these evaluation datasets~\cite{lin2014microsoft,thomee2016yfcc100m} contain rich compositional structure, an important recent work, using $400$ hand-crafted captions with word orders permuted~\cite{thrush2022winoground}, brings to question whether achieving a high performance on retrieval requires compositional understanding. There is, therefore, a need for large-scale benchmark to measure compositionality beyond just word order permutation.

% What's missing:
    % While we have indirect confirmation that these models are capable of some forms of compositionality, such as the impressive ability of DALL-E 2 to combine disparate concepts into coherent scenes, there is a dearth of probing tasks directly investigating whether the learned representations allow for compositionality.
        % Counter-argument: What's wrong with finetuning? Couldn't you perform a linear probe, for instance, on GQA? That should be informative. Why can we also not apply any of the existing linear probes developed for BERT?
            % Answer 1: These models can be used directly as a loss function/evaluation metric without further finetuning. This is why we care about the particular representation space. 
            % Response: Still, linear probing experiments \textit{can} give feedback on what information these representations contain. 
            % Answer 2: Perhaps motivate things from the zero-shot perspective. Why should anyone care about the exact representations?
            % Answer 3: What kinds of confounders do linear probing experiments introduce? The model can pick up on dataset/language biases, for one. I'm sure that there are criticisms of the linear probing set up in both recent vision evaluation work and in the NLP literature.
    % Claim (that needs evidence): Existing benchmarks that allow for zero-shot generalization, such as image classification or retrieval datasets, cannot be used to stress-test compositionality in a directed manner.

% Currently, our insights regarding whether CLIP encodes information for compositionality comes from indirect sources. For instance, while DALL-E 2~\citep{ramesh2022hierarchical}, which uses frozen CLIP text embeddings as its basis, can impressively compose distinct objects, scenes and attributes to generate coherent images, the complexity of its architecture makes it difficult to attribute its success to CLIP representations~\citep{hewitt-liang-2019-designing}. On the other hand, although studies that investigate CLIP's zero-shot performance~\citep{subramanian2022reclip} give direct insights into whether its representations are useful, they fail to stress-test compositionality.


% Bit-flip:
    % We propose a new retrieval benchmark built from VG scene graph annotations that can be used to probe whether the visuo-semantic representation spaces of large pre-trained models allow for compositional reasoning.
    % Our benchmark has two splits for two facets of compositionality: systematicity and productivity. 
    % Why retrieval? 1) Similarity scores are hard to interpret, rank ordering is more interpretable with a carefully designed dataset. 2) Visually evaluating generated images adds a confounding factor (generator) and...human subjectivity?
        % Counterpoint: who is even claiming that raw similarity scores would be a good benchmark?
    % [TODO] We focus on representations; reiterate why.
    
Our paper introduces \name: a new large-scale benchmark to evaluate two important aspects of compositionality: systematicity and productivity (Figure~\ref{fig:pull_figure}). Systematicity measures how well a model is able to represent seen versus unseen atoms and compositions. Productivity measure how well a model is able to represent complex compositions with large number of atoms. We build \name from Visual Genome's scene graphs and region descriptions~\citep{krishnavisualgenome}. To test systematicity, we parse the captions in three popular pretraining datasets, CC-12M~\cite{}, YFCC-15M~\cite{}, and LAION-400M~\cite{}, into scene graphs and use them to create three separate test datasets, containing $385K$, $385K$ and $373K$ image-text pairs. Each corresponding test dataset allows us to test how well a model trained on that pretraining dataset generalizes to novel compositions. Following Morgan's Canon, we additionally generate three more test sets with hard negative captions to ensure we have sufficient empirical evidence for our conclusions. We use GPT-3 to generate the hard negatives and manually verify generation accuracy ($86\%$), leading to $37K$, $34K$, and $30K$ hard negative captions for the three datasets. To test productivity, \name contains 45K image-text pairs with different complexities plus $72K$ hard negative captions with atomic, swapping and negation foils.


%Both compositionality tests require the retrieval dataset to encompass an exhaustive combination of attributes, objects, and relationships; we therefore introduce a set of augmentations which ensure that, for any Visual Genome data point, there exist sufficiently similar images and captions that a model with weaker compositionality would confound with said data point. \textit{More detail about this augmentation?} In contrast to evaluation with generated images and linear probes, which introduce confounding architectures, relying on retrieval from this novel dataset allows us to truly probe the compositionality of the representation space.


Our results find that pretrained vision-language foundation models exhibit little compositionality, neither systematicity nor productivity. We report the following five findings.
First, our systematicity experiments find that models perform similarly regardless of whether the compositions are seen or unseen. This leads us to question the utility of existing datasets for measuring compositionality, leading to the creation of our hard negative test datasets.
Second, tests on the hard negative tests datasets show that Recall@1 performance drops a significant $20\%$ when compositions are unseen.
Third, our productivity experiments show that models performance remains near random chance as the number of atoms in the compositions increase.
Fourth, \rak{TODO: say something about pretraining dataset size}
Fifth and finally, \rak{TODO: say something about model size}

% TODO: results
% How can these findings generalize to 5 years from now?
% a framework for assessing compositionality in multimodal models
% a new image2text & text2image retrieval dataset

==> old/01_introduction_v4.tex <==
\section{Introduction}
Comparative psychology, specifically Morgan's Canon~\cite{morgan1894introduction}, has come to appreciate that human researchers are vulnerable to systematic biases when comparing human and nonhuman intelligence. Understood as an error, Morgan's Canon is the tendency of people to attribute human-like capabilities to non-humans on the basis of insufficient empirical evidence. In an effort to avoid this error in interpreting the emergent machine capabilities~\cite{buckner2019comparative}, this paper focuses on evaluating today's popular vision-language foundation models. Given our learned models' propensity for shortcut learning~\cite{geirhos2020shortcut}, wherein they maximize benchmark performance while failing to generalize to real applications, it is vital that we uncover deficiencies in model behavior. Understanding model behavior is particularly vital for foundation models~\cite{radford2021learning}, which have ubiquitously become the ``foundation'' atop which other models are trained~\cite{conwell2022testing,ramesh2022hierarchical,saharia2022photorealistic}.

% In recent years, vision-language research has been experiencing a shift away from crafting specialized architectures for particular tasks towards the design of task-agnostic models pre-trained with self-supervision on large datasets~(\cite{tan2019lxmert, lu2019vilbert, Zhang_2021_CVPR, Desai_2021_CVPR}). Among these models, CLIP~\cite{radford2021learning}, which learns a shared embedding space for images and text through a contrastive loss, has recently experienced great popularity, with promising use cases beyond standard fine-tuning on downstream tasks, such as zero-shot transfer~\cite{subramanian2022reclip} and automatic caption evaluation~\cite{hessel-etal-2021-clipscore}. As CLIP's applications increase, it becomes more important to understand and evaluate its capabilities.
        
One crucial capability we expect to see in vision-language models is \textit{compositionality}, a fundamental human capability using which people understand new scenes and generate complex sentences~\cite{janssen1997compositionality,hupkes2020compositionality,bottou2014machine}. Compositionality allows us to understand ``the meaning of a whole [a]s a function of the meanings of its [atoms]''~\cite{cresswell1973logics}. For language, these atoms are words that form the sentence while for visual scenes, they are the objects that populate scenes along their attributes, relationships and actions~\cite{krishnavisualgenome,ji2020action}. Compositionality allows people to differentiate between ``TODO'' and ``TODO'' (Figure~\ref{fig:pull_figure}). This capability is hypothesized to partly enable humans' ability to systematically generalize to novel, unseen inputs and can additionally confer beneficial properties such as interpretability or controllability to machine learning models~\cite{lake_ullman_tenenbaum_gershman_2017,bommasani2021opportunities}. 
% Given compositionality's advantages, we investigate whether today's best vision-language models encode necessary information for compositional reasoning.

% We need a paragraph here about why it is hard to measure compositionality today.
While we have indirect confirmation that these models are capable of some forms of compositionality, such as the impressive ability of DALL-E 2 to combine disparate concepts into coherent scenes~\cite{ramesh2022hierarchical}, there is a dearth of probing evaluations directly investigating whether the learned representations allow for compositionality.
These models are trained using web-scraped datasets, comprised of millions of images with their associated text captions~\cite{thomee2016yfcc100m,schuhmann2021laion,sharma2018conceptual} 
%The dominant training paradigm is a contrastive objective~\cite{radford2021learning}; 
and evaluated using image-text retrieval~\cite{jia2021scaling,radford2021learning,Zhang_2021_CVPR}. Although these evaluation datasets~\cite{lin2014microsoft,thomee2016yfcc100m} contain rich compositional structure, an important recent work, using $400$ hand-crafted captions with word orders permuted~\cite{thrush2022winoground}, brings to question whether achieving a high performance on retrieval requires compositional understanding. There is, therefore, a need for large-scale benchmark to measure compositionality beyond just word order permutation.

% What's missing:
    % While we have indirect confirmation that these models are capable of some forms of compositionality, such as the impressive ability of DALL-E 2 to combine disparate concepts into coherent scenes, there is a dearth of probing tasks directly investigating whether the learned representations allow for compositionality.
        % Counter-argument: What's wrong with finetuning? Couldn't you perform a linear probe, for instance, on GQA? That should be informative. Why can we also not apply any of the existing linear probes developed for BERT?
            % Answer 1: These models can be used directly as a loss function/evaluation metric without further finetuning. This is why we care about the particular representation space. 
            % Response: Still, linear probing experiments \textit{can} give feedback on what information these representations contain. 
            % Answer 2: Perhaps motivate things from the zero-shot perspective. Why should anyone care about the exact representations?
            % Answer 3: What kinds of confounders do linear probing experiments introduce? The model can pick up on dataset/language biases, for one. I'm sure that there are criticisms of the linear probing set up in both recent vision evaluation work and in the NLP literature.
    % Claim (that needs evidence): Existing benchmarks that allow for zero-shot generalization, such as image classification or retrieval datasets, cannot be used to stress-test compositionality in a directed manner.

% Currently, our insights regarding whether CLIP encodes information for compositionality comes from indirect sources. For instance, while DALL-E 2~\citep{ramesh2022hierarchical}, which uses frozen CLIP text embeddings as its basis, can impressively compose distinct objects, scenes and attributes to generate coherent images, the complexity of its architecture makes it difficult to attribute its success to CLIP representations~\citep{hewitt-liang-2019-designing}. On the other hand, although studies that investigate CLIP's zero-shot performance~\citep{subramanian2022reclip} give direct insights into whether its representations are useful, they fail to stress-test compositionality.


% Bit-flip:
    % We propose a new retrieval benchmark built from VG scene graph annotations that can be used to probe whether the visuo-semantic representation spaces of large pre-trained models allow for compositional reasoning.
    % Our benchmark has two splits for two facets of compositionality: systematicity and productivity. 
    % Why retrieval? 1) Similarity scores are hard to interpret, rank ordering is more interpretable with a carefully designed dataset. 2) Visually evaluating generated images adds a confounding factor (generator) and...human subjectivity?
        % Counterpoint: who is even claiming that raw similarity scores would be a good benchmark?
    % [TODO] We focus on representations; reiterate why.
    
Our paper introduces \name: a new large-scale benchmark to evaluate two important aspects of compositionality: systematicity and productivity (Figure~\ref{fig:pull_figure}). Systematicity measures how well a model is able to represent seen versus unseen atoms and compositions. Productivity measure how well a model is able to represent complex compositions with large number of atoms. We build \name from Visual Genome's scene graphs and region descriptions~\citep{krishnavisualgenome}. To test systematicity, we parse the captions in three popular pretraining datasets, CC-12M~\cite{}, YFCC-15M~\cite{}, and LAION-400M~\cite{}, into scene graphs and use them to create three separate test datasets, containing $385K$, $385K$ and $373K$ image-text pairs. Each corresponding test dataset allows us to test how well a model trained on that pretraining dataset generalizes to novel compositions. Following Morgan's Canon, we additionally generate three more test sets with hard negative captions to ensure we have sufficient empirical evidence for our conclusions. We use GPT-3 to generate the hard negatives and manually verify generation accuracy ($86\%$), leading to $37K$, $34K$, and $30K$ hard negative captions for the three datasets. To test productivity, \name contains 45K image-text pairs with different complexities plus $72K$ hard negative captions with atomic, swapping and negation foils.


%Both compositionality tests require the retrieval dataset to encompass an exhaustive combination of attributes, objects, and relationships; we therefore introduce a set of augmentations which ensure that, for any Visual Genome data point, there exist sufficiently similar images and captions that a model with weaker compositionality would confound with said data point. \textit{More detail about this augmentation?} In contrast to evaluation with generated images and linear probes, which introduce confounding architectures, relying on retrieval from this novel dataset allows us to truly probe the compositionality of the representation space.


Our results find that pretrained vision-language foundation models exhibit little compositionality, neither systematicity nor productivity. We report the following five findings.
First, our systematicity experiments find that models perform similarly regardless of whether the compositions are seen or unseen. This leads us to question the utility of existing datasets for measuring compositionality, leading to the creation of our hard negative test datasets.
Second, tests on the hard negative tests datasets show that Recall@1 performance drops a significant $20\%$ when compositions are unseen.
Third, our productivity experiments show that models performance remains near random chance as the number of atoms in the compositions increase.
Fourth, \rak{TODO: say something about pretraining dataset size}
Fifth and finally, \rak{TODO: say something about model size}

% TODO: results
% How can these findings generalize to 5 years from now?
% a framework for assessing compositionality in multimodal models
% a new image2text & text2image retrieval dataset

==> old/01_introduction_v5.tex <==
\section{Introduction}
Compositionality, that ``the meaning of the whole is a function of the meanings of its parts''~\cite{cresswell1973logics}, is held to be a key characteristic of human intelligence, enabling people to reason, communicate, and plan~\cite{bommasani2021opportunities}. A characteristic so fundamental that it underlies the human capability to understand new scenes and generate complex sentences~\cite{janssen1997compositionality,hupkes2020compositionality,bottou2014machine}. For language, these parts are words that form the sentence while for visual scenes, they are the objects along with their attributes, relationships, and actions~\cite{krishnavisualgenome,ji2020action}.  
Compositionality allows people to differentiate between ``Yellow vase on top of a black television'' and ``Black television on top of a yellow vase''.
Despite its importance in both vision and in language, we don't yet have a large-scale benchmark to evaluate whether our community's pervasive vision-language foundation models can reason compositionally. Understanding model behavior is particularly vital for foundation models~\cite{radford2021learning}, which have ubiquitously become the ``foundation'' atop which other models are trained~\cite{conwell2022testing,ramesh2022hierarchical,saharia2022photorealistic}.

% We need a paragraph here about why it is hard to measure compositionality today.
While we have indirect confirmation that these models are capable of some forms of compositionality, such as the impressive ability of DALL-E 2 to combine disparate concepts into coherent scenes~\cite{ramesh2022hierarchical}, there is a dearth of probing evaluations directly investigating whether the learned representations allow for compositionality.
These models are trained using web-scraped datasets, comprised of millions of images with their associated text captions~\cite{thomee2016yfcc100m,schuhmann2021laion,sharma2018conceptual} 
%The dominant training paradigm is a contrastive objective~\cite{radford2021learning}; 
and evaluated using image-text retrieval~\cite{jia2021scaling,radford2021learning,Zhang_2021_CVPR}. Although these evaluation datasets~\cite{lin2014microsoft,thomee2016yfcc100m} contain rich compositional structure, an important recent work, using $400$ hand-crafted captions with word orders permuted~\cite{thrush2022winoground}, brings to question whether achieving a high performance on retrieval requires compositional understanding. There is, therefore, a need for large-scale benchmark to measure compositionality beyond just word order permutation.




% Bit-flip:
    % We propose a new retrieval benchmark built from VG scene graph annotations that can be used to probe whether the visuo-semantic representation spaces of large pre-trained models allow for compositional reasoning.
    % Our benchmark has two splits for two facets of compositionality: systematicity and productivity. 
    % Why retrieval? 1) Similarity scores are hard to interpret, rank ordering is more interpretable with a carefully designed dataset. 2) Visually evaluating generated images adds a confounding factor (generator) and...human subjectivity?
        % Counterpoint: who is even claiming that raw similarity scores would be a good benchmark?
    % [TODO] We focus on representations; reiterate why.
    
Our paper introduces \name{}: a new large-scale benchmark to evaluate two important aspects of compositionality: systematicity and productivity (Figure~\ref{fig:pull_figure}). Systematicity measures how well a model is able to represent seen versus unseen atoms and compositions. Productivity measures how well a model is able to represent complex compositions with a large number of atoms. We build \name{} from Visual Genome's scene graphs and region descriptions~\cite{krishnavisualgenome}. To test systematicity, we parse the captions in three popular training datasets, CC-12M~\cite{changpinyo2021conceptual}, YFCC-15M~\cite{thomee2016yfcc100m}, and LAION-400M~\cite{schuhmann2021laion}, into scene graphs and use them to create three separate test datasets, containing $385K$, $385K$ and $373K$ image-text pairs respectively. Each corresponding test dataset allows us to test how well a model trained on that training dataset generalizes to novel compositions. We additionally generate three more test sets with hard negative captions to ensure we have sufficient empirical evidence for our conclusions. We use GPT-3 to generate the hard negatives and manually verify generation accuracy ($86\%$), leading to $37K$, $34K$, and $30K$ hard negative captions for the three datasets. To test productivity, \name{} contains 45K image-text pairs with different complexities plus $72K$ hard negative captions with atomic, swapping and negation foils. 

Our results find that vision-language foundation models exhibit little compositionality, neither systematicity nor productivity. We report the following five findings.
First, our systematicity experiments find that models perform similarly regardless of whether the compositions are seen or unseen. This leads us to question the utility of existing datasets for measuring compositionality, leading to the creation of our hard negative test datasets.
Second, tests on the hard negative tests datasets show that Recall@1 performance drops a significant $20\%$ when compositions are unseen.
Third, our productivity experiments show that models performance remains near random chance as the number of atoms in the compositions increase.
Fourth, \rak{TODO: say something about training dataset size}
Fifth and finally, \rak{TODO: say something about model size}

% TODO: results
% How can these findings generalize to 5 years from now?
% a framework for assessing compositionality in multimodal models
% a new image2text & text2image retrieval dataset

==> old/01_introduction_v6.tex <==

\input{figures/pull_figure}

\section{Introduction}
Compositionality, that ``the meaning of the whole is a function of the meanings of its parts''~\cite{cresswell1973logics}, is held to be a key characteristic of human intelligence, enabling people to reason, communicate, and plan~\cite{bommasani2021opportunities}. Compositional reasoning underlies the human capability to understand new scenes and generate complex sentences~\cite{janssen1997compositionality,hupkes2020compositionality,bottou2014machine}. In language, the whole is a sentence, made up of words, while in visual scenes, the parts are objects, along with their attributes, relationships, and actions~\cite{krishnavisualgenome,ji2020action}.  
%Compositionality allows people to differentiate between ``Yellow vase on top of a black television'' and ``Black television on top of a yellow vase''.
Despite its importance in both vision and language, the vision and language research community lacks a large-scale benchmark to evaluate whether pretrained vision-language models can reason compositionally.
These models are trained using web-scraped datasets, comprising millions of images with their associated text captions~\cite{thomee2016yfcc100m,schuhmann2021laion,sharma2018conceptual}, and applied for tasks like retrieval, text-to-image generation, and open-vocabulary classification.
Especially as these pretrained models become ubiquitous ``foundations'' for other models~\cite{bommasani2021opportunities,conwell2022testing,ramesh2022hierarchical,saharia2022photorealistic}, it is critical to understand their compositional abilities.

% We need a paragraph here about why it is hard to measure compositionality today.
While there is indirect evidence that vision and language models are capable of some forms of compositionality (\eg the impressive ability of DALL-E 2 to combine disparate concepts into coherent scenes~\cite{ramesh2022hierarchical}), there is a lack of probing evaluations that directly investigate whether vision and language models learn representations enabling compositional behavior.
% allow for compositionality.
%The dominant training paradigm is a contrastive objective~\cite{radford2021learning}; 
Previous work has evaluated these models using image-text retrieval~\cite{jia2021scaling,radford2021learning,Zhang_2021_CVPR}. Although these retrieval datasets~\cite{lin2014microsoft,thomee2016yfcc100m} contain some compositional structure, they do not provide controlled sets of negatives for evaluation. Recent work, which uses $800$ hand-crafted negative captions with word orders permuted~\cite{thrush2022winoground}, questions if achieving a high performance on retrieval requires compositional understanding. There is, therefore, a need for a large-scale benchmark to measure compositionality with controlled negatives, extending beyond just word order permutation~\cite{thrush2022winoground}.

% compositional structure, recent work using $800$ hand-crafted captions with word orders permuted~\cite{thrush2022winoground} brings to question whether achieving a high performance on retrieval requires compositional understanding. There is, therefore, a need for a large-scale benchmark to measure compositionality beyond just word order permutation.

    
    % Why retrieval? 1) Similarity scores are hard to interpret, rank ordering is more interpretable with a carefully designed dataset. 2) Visually evaluating generated images adds a confounding factor (generator) and...human subjectivity?
        % Counterpoint: who is even claiming that raw similarity scores would be a good benchmark?
    % [TODO] We focus on representations; reiterate why.
    
We introduce \nameemoji{} (Compositional REPresentation Evaluation): a new large-scale benchmark to evaluate two important aspects of compositionality: \textit{systematicity} and \textit{productivity} (Figure~\ref{fig:pull_figure}). Systematicity measures how well a model is able to represent seen versus unseen \textit{atoms} and their compositions. Productivity measures how well a model is able to represent instances with increasing complexity. \name{} uses Visual Genome's scene graph representation as the compositionality language~\cite{krishnavisualgenome}.

To test systematicity, we parse the captions in three popular training datasets, CC-12M~\cite{changpinyo2021conceptual}, YFCC-15M~\cite{thomee2016yfcc100m}, and LAION-400M~\cite{schuhmann2021laion}, into scene graphs and use them to create three separate retrieval test sets, containing $385K$, $385K$ and $373K$ image-text pairs respectively. Each test dataset allows us to test how well a model trained on that dataset generalizes to novel atoms and compositions. These datasets, unfortunately, contain instances in the retrieval set that are considered negatives but might be unintended positives, resulting in inaccurate results. For example, the caption ``food on a black television'' is an unintended positive for an image containing a ``crepe on a skillet''. 

Therefore, we additionally generate three more retrieval sets with hard negative captions to ensure we have sufficient empirical evidence for our conclusions, leading to $237K$, $210K$ and $178K$ hard negative captions for the three datasets. To test productivity, \name{} contains $17K$ image-text pairs with different complexities plus $246K$ hard negative captions with atomic, swapping, and negation foils. We generate the ground-truth image-text pairs for productivity using templates and GPT-3~\cite{brown2020language}, and manually verify them as having an annotation accuracy of $86\%$.

Overall, our results conclude that vision-language foundation models exhibit little compositionality, neither systematicity nor productivity. We report the following six findings.
First, our systematicity experiments find that models' performance consistently drops between splits featuring seen and unseen compositions. Secondly, this drop is most pronounced for models trained on LAION-400M, with up to a $8\%$ decrease in Recall@1. Third, our productivity experiments indicate that models' ability to discern hard negatives decays with increased caption complexity. Fourth, we find that training set size has no effect on this observation. Fifth, we find no trends relating compositionality to model size. Finally, we find that models' ranking on zero-shot ImageNet classification correlates with their compositionality.
% TODO: results
% How can these findings generalize to 5 years from now?
% a framework for assessing compositionality in multimodal models
% a new image2text & text2image retrieval dataset

==> old/02_related_work_v1.tex <==
\section{Related Work}
\textbf{Image-Text Pretraining} Open with a short reference to LXMERT/ViLBERT type V+L models before referencing CLIP's great success. This section will provide an overview of CLIP's various applications. This will be split into three: its strong performance as a feature extractor in downstream tasks, its ability to be more creatively incorporated into architectures and evaluation protocols and finally how its representations enable zero-shot task performance on a variety of problems. These examples will be followed by different approaches inspired by CLIP, with short descriptions of how they differ from it.

\textbf{Compositionality:} This section has two main goals: Providing a definition of compositionality grounded in the linguistics literature and situating our work within a pre-existing line of work on evaluating compositionality for deep learning models. 

\textbf{BERTology}: Situate our work in a parallel line of work evaluating large pretrained models. Short examples on both the NLP and the Computer Vision side. Emphasize the fact that while our work will help better understand CLIP-like models, its emphasis is evaluation. Further describe how the debate on the use probing classifiers in BERTology informs our decision to use retrieval zero-shot to evaluate models.




==> old/02_related_work_v2.tex <==
Comparative psychology, specifically Morgan's Canon~\cite{morgan1894introduction}, has come to appreciate that human researchers are vulnerable to systematic biases when comparing human and nonhuman intelligence. Understood as an error, Morgan's Canon is the tendency of people to attribute human-like characteristics to non-humans on the basis of insufficient empirical evidence. In an effort to avoid this error in interpreting the emergent machine capabilities~\cite{buckner2019comparative}, this paper focuses on evaluating today's popular vision-language foundation models. Given our learned models' propensity for shortcut learning~\cite{geirhos2020shortcut}, wherein they maximize benchmark performance while failing to generalize to real applications, it is vital that we uncover deficiencies in model behavior. Understanding model behavior is particularly especially for foundation models, such as CLIP~\cite{radford2021learning}, which has ubiquitously become the ``foundation'' atop which other models are trained~\cite{conwell2022testing,ramesh2022hierarchical,saharia2022photorealistic}.


% paragraph about why measuring compositionality is hard.
Existing benchmarks used to evaluate vision-language models are insufficient for evaluating the emergence of compositional reasoning. These models are trained using web-scraped datasets, comprised of millions of images with their associated text captions~\cite{thomee2016yfcc100m,schuhmann2021laion,sharma2018conceptual}. The dominant training paradigm is a contrastive objective~\cite{radford2021learning}; the resulting model are evaluated using image-text retrieval over these large datasets~\cite{jia2021scaling,radford2021learning,Zhang_2021_CVPR}. Although these datasets contain rich compositional structure, we show that achieve a high performance on retrieval doesn't require compositionality. A test for compositional understanding requires images with captions containing similar words but different compositional rules (see Figure~\ref{fig:pull_figure}). Noticing this deficiency, important recent work has introduced a small test set with $400$ hand-crafted captions with word orders permuted~\cite{thrush2022winoground}. Although valuable, there is a need for larger benchmarks that test for a more ... \rak{need to say that we are different from winoground.}.

==> old/02_related_work_v3.tex <==
\section{Related Work}
We situate our work amongst others that evaluate contrastive vision-language foundation models. Specifically, we measure visio-linguistic compositionality. In other to do so, we generate hard negatives using GPT-3.

\noindent\textbf{Contrastive Image-Text Pretraining} 
The recently released contrastively trained CLIP model~\cite{radford2021learning} has catalyzed a wide array of work at the intersection of Computer Vision and Natural Language Processing. Since its release, in addition to being used successfully as a feature extractor for various vision and language tasks~\cite{shen2022how}, CLIP has enabled several tasks, ranging from semantic segmentation to image captioning, to be solved in a zero-shot manner~\cite{radford2021learning, li2022languagedriven, tewel2021zero, subramanian2022reclip, https://doi.org/10.48550/arxiv.2109.02748, pmlr-v168-cui22a}, has been used as a loss function within image synthesis applications~\cite{https://doi.org/10.48550/arxiv.2112.05744, Patashnik_2021_ICCV, xu2022ppe, Li_2022_CVPR, zhou2021lafite, Jain_2021_ICCV}, acted as an automated evaluation metric~\cite{park2021benchmark, hessel-etal-2021-clipscore} and has been incorporated into architectures for various tasks including dense prediction and video summarization~\cite{9880269, rao2021denseclip, cosnet2022cvpr, shridhar2021cliport, https://doi.org/10.48550/arxiv.2107.00650, https://doi.org/10.48550/arxiv.2201.06696}. This success has also encouraged the design of other contrastive vision and language pretraining algorithms for image~\cite{li2021align, https://doi.org/10.48550/arxiv.2205.14459, https://doi.org/10.48550/arxiv.2204.07441,https://doi.org/10.48550/arxiv.2203.00048, li-etal-2022-unimo,yu2022coca, yang2022vision,https://doi.org/10.48550/arxiv.2112.04482, li2022blip} and video domains~\cite{9878891, https://doi.org/10.48550/arxiv.2109.08472, xu-etal-2021-videoclip}. Given the prevalence of CLIP-like models, our work evaluates how well CLIP is able to understand the compositional nature of both vision and language.

\noindent\textbf{Evaluating learned representations} By analyzing the properties of pretrained representations, our work continues a tradition of research in Natural Language Processing~\cite{rogers-etal-2020-primer, jawahar-etal-2019-bert, tenney-etal-2019-bert, webson-pavlick-2022-prompt, hessel-schofield-2021-effective, pham-etal-2021-order} and Computer Vision~\cite{li-etal-2020-bert-vision, rosch-libovicky-2022-probing, milewski-etal-2022-finding, https://doi.org/10.48550/arxiv.2206.07835, https://doi.org/10.48550/arxiv.2204.03162, frank-etal-2021-vision} that investigates characteristics of large pretrained models themselves rather than their performance on downstream tasks. 
Our decision to use retrieval for zero-shot evaluation, in particular, was influenced by work seeking to avoid limitations of the probing classifier paradigm~\cite{hewitt-liang-2019-designing, belinkov-2022-probing} by using evaluation procedures that don't require learning additional parameters~\cite{https://doi.org/10.48550/arxiv.2104.03514, https://doi.org/10.48550/arxiv.2011.12073,zhou-srikumar-2021-directprobe}. 

\noindent\textbf{Compositionality}
% Define compositionality in the traditional sense and describe why it is important for vision
    % Examples of general papers
    % For the latter half, foundation models paper and visual genome
Compositionality, that "the meaning of the whole is a function of the meanings
of its parts"~\cite{cresswell1973logics}, is held to be a key component of intelligence, enabling humans to reason and  plan~\cite{bommasani2021opportunities} and to comprehend an infinite number of scenes and utterances~\cite{lake_ullman_tenenbaum_gershman_2017}. For an AI model, compositionality would not only allow for systematic, combinatorial generalization, but would also confer benefits such as controllability~\cite{bommasani2021opportunities}. This promise has prompted a wealth of work on both designing compositional models~\cite{higgins2017scan, https://doi.org/10.48550/arxiv.1511.02799, https://doi.org/10.48550/arxiv.1803.03067} and evaluating them~\cite{hudson2018gqa, GrundeMcLaughlin2021AGQA, lake2018generalization, suhr-etal-2019-corpus}. 

In our work, we focus on two aspects of compositionality: systematicity, the ability to comprehend novel combinations of known components, and productivity, the ability to understand inputs of greater length or complexity than those seen before~\cite{hupkes2020compositionality}. While there exists a plethora of benchmarks for systematic generalization within Computer Vision~\cite{https://doi.org/10.48550/arxiv.1612.06890, bahdanau2019closure, bogin-etal-2021-covr, GrundeMcLaughlin2021AGQA} and Machine Learning in general~\cite{lake2018generalization, 10.5555/3495724.3497391, keysers2020measuring}, the subject has been less explored for pretrained vision-language models due to the models using different training sets. To address this, CREPE provides three different datasets to evaluate the compositional generalization of vision-language models trained on the commonly used Conceptual Captions 12M~\cite{changpinyo2021conceptual}, YFCC 15M~\cite{thomee2016yfcc100m, radford2021learning} and LAION400~\cite{schuhmann2021laion}. Productivity, on the other hand, has been studied less overall~\cite{lake2018generalization, 10.5555/3495724.3497391, hupkes2020compositionality, GrundeMcLaughlin2021AGQA}. CREPE evaluates the productivity of vision-language models with a image-text retrieval dataset featuring captions of varying complexity.
\noindent\textbf{Evaluation with hard negatives}
% Overview evaluating V+L models with hard negatives
Like us, past work for the evaluation of vision-language models has commonly designed tasks featuring hard negatives to target particular model capabilities while overcoming the limitations of prior evaluation tasks. 
% Overview of atomic foils
    % FOIL-It, BISON, Probing Image-Language Transformers for Word Understanding, Cops-Ref (referring expressions, minor degree of productivity), COVR, Exposing the Limits of Video-Text, VALSE, Image Retrieval from Contextual Descriptions, Seeing Past Words (maybe))
Using atomic foils that replace an atom in the image or text with a distractor has been the most common strategy~\cite{shekhar-etal-2017-foil, https://doi.org/10.48550/arxiv.1901.06595, https://doi.org/10.48550/arxiv.2106.09141, https://doi.org/10.48550/arxiv.2003.00403, bogin-etal-2021-covr, park-etal-2022-exposing, parcalabescu-etal-2022-valse}.
    % Special note of COVR, VALSE and the Video Contrast Set paper. Contrast based on productivity (special note on Cops-Ref)
Park \textit{et al.}~\cite{park-etal-2022-exposing} evaluate video-text models with hard-negatives targeting verbs and person entities.
COVR~\cite{bogin-etal-2021-covr} evaluates the systematic generalization of vision-language models on a question answering task where the models are input a set of distractor images. VALSE~\cite{parcalabescu-etal-2022-valse}, finally, provides a zero-shot evaluation of pretrained vision-language models with hard negatives targeting linguistic phenomena such as existence, cardinality and the recognition of actions and spatial relationships.
% Overview of swapping-based
    % Less prevalent. Words Aren't Enough (referring exp), When and Why (OpenReview), Winoground, VALSE (actions)
    % Key difference: Emphasis on systematic generalization and productivity
Another strategy has been to swap atoms within a caption to generate hard-negatives testing whether models behave like bag-of-words models~\cite{akula-etal-2020-words, parcalabescu-etal-2022-valse, thrush2022winoground, https://doi.org/10.48550/arxiv.2210.01936}. Winoground~\cite{thrush2022winoground} and the contemporary work of Yuksekgonul \textit{et al.}~\cite{https://doi.org/10.48550/arxiv.2210.01936}, by generating swapping-based negatives to assess the compositionality of pretrained vision-language models in a zero-shot manner, are the most similar to us. Our dataset CREPE distinguishes itself from past work using atomic foils or swapping-based negatives by evaluating the systematic generalization and productivity (which has been particularly understudied) of pretrained vision-language models in a zero-shot manner. \omer{Is a subsection on negation necessary? Also, I don't think that we should add the hard negative papers from the OpenReview paper as they're all focused on training} 

% Overview of negation-based:
    % This section could use more papers. Write this as a note

==> old/02_related_work_v4.tex <==
\section{Related Work}
We situate our work amongst others that evaluate contrastive vision-language foundation models. Specifically, we measure visio-linguistic compositionality. In other to do so, we generate hard negatives using GPT-3.

\noindent\textbf{Evaluating learned representations} By analyzing the properties of pretrained representations, our work continues a tradition of research in Computer Vision~\cite{li-etal-2020-bert-vision, rosch-libovicky-2022-probing, milewski-etal-2022-finding, https://doi.org/10.48550/arxiv.2206.07835, https://doi.org/10.48550/arxiv.2204.03162, frank-etal-2021-vision} and Natural Language Processing~\cite{rogers-etal-2020-primer, jawahar-etal-2019-bert, tenney-etal-2019-bert, webson-pavlick-2022-prompt, hessel-schofield-2021-effective, pham-etal-2021-order} that probes characteristics of large pretrained representations themselves rather than their performance on downstream tasks. 
Instead of learning probes, we use retrieval for zero-shot evaluation in order to avoid scenarios where the learned probe compensates for the characteristics deficient in the original representations~\cite{hewitt-liang-2019-designing,belinkov-2022-probing}. We draw on recent methods that design probes which don't require learning additional parameters~\cite{https://doi.org/10.48550/arxiv.2104.03514,https://doi.org/10.48550/arxiv.2011.12073,zhou-srikumar-2021-directprobe}.

\noindent\textbf{Contrastive Image-Text Pretraining} 
The recently released contrastively trained CLIP model~\cite{radford2021learning} has catalyzed a wide array of work at the intersection of Computer Vision and Natural Language Processing. Since its release, CLIP has enabled several tasks, ranging from semantic segmentation to image captioning, many of which have now produce remarkable zero-shot capability~\cite{radford2021learning,li2022languagedriven,tewel2021zero, subramanian2022reclip,https://doi.org/10.48550/arxiv.2109.02748,pmlr-v168-cui22a}. CLIP has been used as a loss function within image synthesis applications~\cite{https://doi.org/10.48550/arxiv.2112.05744, Patashnik_2021_ICCV, xu2022ppe, Li_2022_CVPR, zhou2021lafite, Jain_2021_ICCV}, acted as an automated evaluation metric~\cite{park2021benchmark, hessel-etal-2021-clipscore}, used successfully as a feature extractor for various vision and language tasks~\cite{shen2022how}, and incorporated into architectures for various tasks including dense prediction and video summarization~\cite{9880269,rao2021denseclip,cosnet2022cvpr,shridhar2021cliport,https://doi.org/10.48550/arxiv.2107.00650,https://doi.org/10.48550/arxiv.2201.06696}. This success has also encouraged the design of other contrastive vision and language pretraining algorithms for image~\cite{li2021align,https://doi.org/10.48550/arxiv.2205.14459,https://doi.org/10.48550/arxiv.2204.07441,https://doi.org/10.48550/arxiv.2203.00048,li-etal-2022-unimo,yu2022coca,yang2022vision,https://doi.org/10.48550/arxiv.2112.04482,li2022blip} and video domains~\cite{9878891,https://doi.org/10.48550/arxiv.2109.08472,xu-etal-2021-videoclip}. Given the prevalence of CLIP-like models, our work evaluates how well different CLIP models capture a fundamental property present in human vision and natural language: compositionality.


\noindent\textbf{Compositionality}
% Define compositionality in the traditional sense and describe why it is important for vision
    % Examples of general papers
    % For the latter half, foundation models paper and visual genome
% Compositionality, that ``the meaning of the whole is a function of the meanings of its parts''~\cite{cresswell1973logics}, is held to be a key characteristic of human intelligence, enabling people to reason, communicate, and plan~\cite{bommasani2021opportunities}. 
Compositionality allows us to comprehend an infinite number of scenes and utterances~\cite{lake_ullman_tenenbaum_gershman_2017}. For an AI model, compositionality would not only allow for systematic, combinatorial generalization, but would also confer benefits such as controllability~\cite{bommasani2021opportunities}. This promise has prompted a wealth of work on both designing compositional models~\cite{higgins2017scan,https://doi.org/10.48550/arxiv.1511.02799,https://doi.org/10.48550/arxiv.1803.03067} and evaluating them~\cite{hudson2018gqa,GrundeMcLaughlin2021AGQA,lake2018generalization,suhr-etal-2019-corpus,gandhi2022measuring}. 
In our work, we focus on two aspects of compositionality: systematicity, the ability to comprehend novel combinations of known components, and productivity, the ability to understand inputs of greater complexity than those seen before~\cite{hupkes2020compositionality}. While there exists a plethora of benchmarks for systematic generalization within Computer Vision~\cite{https://doi.org/10.48550/arxiv.1612.06890,bahdanau2019closure,bogin-etal-2021-covr,GrundeMcLaughlin2021AGQA} and Machine Learning in general~\cite{lake2018generalization,10.5555/3495724.3497391,keysers2020measuring}, the subject has been almost unexplored for pretrained vision-language models, largely due to lack of benchmarks complementary to the different large-scale training datasets. To address this, \name{} provides a benchmark with three different datasets to evaluate the compositional generalization of vision-language models trained on the commonly used CC-12M~\cite{changpinyo2021conceptual}, YFCC-15M~\cite{thomee2016yfcc100m, radford2021learning} and LAION-400~\cite{schuhmann2021laion}. Productivity, on the other hand, has been studied only for specialized tasks~\cite{GrundeMcLaughlin2021AGQA} or toy domains~\cite{lake2018generalization,10.5555/3495724.3497391, hupkes2020compositionality}. \name{} evaluates the productivity with using the image-text retrieval task featuring captions of varying compositional complexity.

\noindent\textbf{Evaluation with hard negatives}
% Overview evaluating V+L models with hard negatives
Like us, past work evaluating vision-language models has commonly designed tasks featuring hard negatives to target particular model capabilities while overcoming the limitations of prior evaluation tasks. 
% Overview of atomic foils
    % FOIL-It, BISON, Probing Image-Language Transformers for Word Understanding, Cops-Ref (referring expressions, minor degree of productivity), COVR, Exposing the Limits of Video-Text, VALSE, Image Retrieval from Contextual Descriptions, Seeing Past Words (maybe))
Using atomic foils that replace an atom in the image or text with a distractor has been the most common strategy~\cite{shekhar-etal-2017-foil,https://doi.org/10.48550/arxiv.1901.06595,https://doi.org/10.48550/arxiv.2106.09141,https://doi.org/10.48550/arxiv.2003.00403,bogin-etal-2021-covr, park-etal-2022-exposing, parcalabescu-etal-2022-valse}.
    % Special note of COVR, VALSE and the Video Contrast Set paper. Contrast based on productivity (special note on Cops-Ref)
Park \textit{et al.}~\cite{park-etal-2022-exposing} evaluate video-text models with hard-negatives targeting verbs and person entities.
COVR~\cite{bogin-etal-2021-covr} evaluates the systematic generalization on a question answering task with distractor images. VALSE~\cite{parcalabescu-etal-2022-valse}, provides a zero-shot evaluation of pretrained vision-language models with hard negatives targeting linguistic phenomena such as existence, cardinality and the recognition of actions and spatial relationships.
% Overview of swapping-based
    % Less prevalent. Words Aren't Enough (referring exp), When and Why (OpenReview), Winoground, VALSE (actions)
    % Key difference: Emphasis on systematic generalization and productivity
Another strategy has been to swap atoms within a caption to generate hard-negatives testing whether models behave like bag-of-words models~\cite{akula-etal-2020-words, parcalabescu-etal-2022-valse, thrush2022winoground, https://doi.org/10.48550/arxiv.2210.01936}. Winoground~\cite{thrush2022winoground} and the contemporary work of Yuksekgonul \textit{et al.}~\cite{https://doi.org/10.48550/arxiv.2210.01936}, by generating swapping-based negatives to assess the compositionality of pretrained vision-language models in a zero-shot manner, are the most similar to us. Our dataset CREPE distinguishes itself from past work using atomic foils or swapping-based negatives by evaluating the systematic generalization and productivity (which has been particularly understudied) of pretrained vision-language models in a zero-shot manner. \omer{Is a subsection on negation necessary? Also, I don't think that we should add the hard negative papers from the OpenReview paper as they're all focused on training} 

% Overview of negation-based:
    % This section could use more papers. Write this as a note

==> old/02_related_work_v5.tex <==
\section{Related Work}
Our work lies within the field of evaluating foundation models. Specifically, we measure visio-linguistic compositionality. To do so, we create a retrieval benchmark with hard negatives.

\noindent\textbf{Contrastive Image-Text Pretraining} 
The recently released contrastively trained CLIP model~\cite{radford2021learning} has catalyzed a wide array of work at the intersection of Computer Vision and Natural Language Processing. Since its release, CLIP has enabled several tasks, ranging from semantic segmentation to image captioning, many of which have remarkable zero-shot capability~\cite{radford2021learning,li2022languagedriven,tewel2021zero, subramanian2022reclip,https://doi.org/10.48550/arxiv.2109.02748,pmlr-v168-cui22a}. CLIP has been used as a loss function within image synthesis applications~\cite{https://doi.org/10.48550/arxiv.2112.05744, Patashnik_2021_ICCV, xu2022ppe, Li_2022_CVPR, zhou2021lafite, Jain_2021_ICCV}, acted as an automated evaluation metric~\cite{park2021benchmark, hessel-etal-2021-clipscore}, used successfully as a feature extractor for various vision and language tasks~\cite{shen2022how}, and incorporated into architectures for various tasks including dense prediction and video summarization~\cite{9880269,rao2021denseclip,cosnet2022cvpr,shridhar2021cliport,https://doi.org/10.48550/arxiv.2107.00650,https://doi.org/10.48550/arxiv.2201.06696}. This success has also encouraged the design of other contrastive vision and language pretraining algorithms for image~\cite{li2021align,https://doi.org/10.48550/arxiv.2205.14459,https://doi.org/10.48550/arxiv.2204.07441,https://doi.org/10.48550/arxiv.2203.00048,li-etal-2022-unimo,yu2022coca,yang2022vision,https://doi.org/10.48550/arxiv.2112.04482,li2022blip} and video domains~\cite{9878891,https://doi.org/10.48550/arxiv.2109.08472,xu-etal-2021-videoclip}. Given the prevalence of CLIP-like models, our work evaluates how well different CLIP models capture a fundamental property present in human vision and natural language: compositionality.


%=====================
% SYSTEMATICITY FIGURE
\input{figures/systematicity_figure}
%=====================

\noindent\textbf{Compositionality}
% Define compositionality in the traditional sense and describe why it is important for vision
    % Examples of general papers
    % For the latter half, foundation models paper and visual genome
Compositionality allows us to comprehend an infinite number of scenes and utterances~\cite{lake_ullman_tenenbaum_gershman_2017}. For an AI model, compositionality would not only allow for systematic, combinatorial generalization, but would also confer benefits such as controllability~\cite{bommasani2021opportunities}. This promise prompted a wealth of work on both designing~\cite{higgins2017scan,https://doi.org/10.48550/arxiv.1511.02799,https://doi.org/10.48550/arxiv.1803.03067} and evaluating ~\cite{hudson2018gqa,GrundeMcLaughlin2021AGQA,lake2018generalization,suhr-etal-2019-corpus,gandhi2022measuring} compositional models. 
In our work, we focus on two aspects of compositionality: systematicity and productivity.
%, the ability to comprehend novel combinations of known components, 
%, the ability to understand inputs of greater complexity than those seen before~\cite{hupkes2020compositionality}. 
While there is a plethora of benchmarks for systematic generalization within Computer Vision~\cite{https://doi.org/10.48550/arxiv.1612.06890,bahdanau2019closure,bogin-etal-2021-covr,GrundeMcLaughlin2021AGQA} and Machine Learning~\cite{lake2018generalization,10.5555/3495724.3497391,keysers2020measuring}, the subject has been almost unexplored for vision-language models, largely due to lack of benchmarks complementary to the different large-scale training datasets. To address this, \name{} provides a benchmark with three different datasets to evaluate the compositional generalization of vision-language models.
%trained on the commonly used CC-12M~\cite{changpinyo2021conceptual}, YFCC-15M~\cite{thomee2016yfcc100m, radford2021learning} and LAION-400M~\cite{schuhmann2021laion}. 
Productivity, on the other hand, has been studied only for specialized tasks~\cite{GrundeMcLaughlin2021AGQA} or toy domains~\cite{lake2018generalization,10.5555/3495724.3497391, hupkes2020compositionality}. \name{} evaluates productivity by using an image-text retrieval task featuring captions of varying compositional complexity.


\noindent\textbf{Evaluation with hard negatives}
% Overview evaluating V+L models with hard negatives
Like us, past work evaluating models has commonly designed tasks featuring hard negatives to isolate particular model capabilities while overcoming the limitations of prior evaluation tasks. 
% Overview of atomic foils
    % FOIL-It, BISON, Probing Image-Language Transformers for Word Understanding, Cops-Ref (referring expressions, minor degree of productivity), COVR, Exposing the Limits of Video-Text, VALSE, Image Retrieval from Contextual Descriptions, Seeing Past Words (maybe))
Using atomic foils that replace an atom in the image or text with a distractor has been the most common strategy~\cite{shekhar-etal-2017-foil,https://doi.org/10.48550/arxiv.1901.06595,https://doi.org/10.48550/arxiv.2106.09141,https://doi.org/10.48550/arxiv.2003.00403,bogin-etal-2021-covr, park-etal-2022-exposing, parcalabescu-etal-2022-valse}.
    % Special note of COVR, VALSE and the Video Contrast Set paper. Contrast based on productivity (special note on Cops-Ref)
Notably, Park \textit{et al.}~\cite{park-etal-2022-exposing} targets verbs and person entities in videos;
COVR~\cite{bogin-etal-2021-covr} studies question answering with distractor images; VALSE~\cite{parcalabescu-etal-2022-valse} targets linguistic phenomena such as existence, cardinality and the recognition of actions and spatial relationships.
% Overview of swapping-based
    % Less prevalent. Words Aren't Enough (referring exp), When and Why (OpenReview), Winoground, VALSE (actions)
    % Key difference: Emphasis on systematic generalization and productivity
Another strategy has been to swap atoms within a caption to test whether models behave akin to a bag-of-words~\cite{akula-etal-2020-words,parcalabescu-etal-2022-valse,thrush2022winoground}. In particular, Winoground~\cite{thrush2022winoground} introduces a set of $800$ human edited negatives to evaluate compositionality; it is the closest related work to us. We complement Winoground by scaling it up by three orders of magnitude, by decomposing compositionality into systematicity and productivity, and by studying a variety of different types of hard negatives.

==> old/03_compositionality_v1.tex <==
\section{Compositional evaluation}


Though the \textit{principle} of compositionality is well-defined, we echo the warning of Hupkes \textit{et al.}~\cite{hupkes2020compositionality} that this principle is ``formally vacuous'' if the syntax and semantics of the composed language are not established. Additionally, once a compositional language is established, it is necessary to define what behaviors to expect from a model that achieves comprehension of said language, as well as how to empirically measure those behaviors. We therefore use this section to define the language underlying our compositional evaluation; describe \textit{what} aspects of compositionality we evaluate; and explain \textit{how} we evaluate them via retrieval. 

\subsection{Compositional language of visual concepts}
% We are primarily concerned with a language of visual concepts, particularly as expressed by the images and corresponding scene graphs of Visual Genome. Accordingly, an \textit{atom} is defined a particular node in a Visual Genome scene graph. These are subdivided into \textit{objects}, \textit{relationships}, and \textit{attributes}. The compositional functions correspond to connection between scene graph nodes in Visual Genome: namely, the semantic attachment of attribute to objects (``black dog”), and the attachment of two objects via a relationship (``man hugs child”). On top of this, our experiments also incorporate the attachment of a negation term onto any atom (``not black").
To evaluate vision-language models in particular, we find that a composition language consisting of visual concepts is an appropriate foundation. We particularly focus on the vocabulary and compositions of scene graph image annotations. Accordingly, an \textit{atom} $A$ is defined as a singular visual concept, corresponding to a single scene graph node. Atoms are subcategorized into \textit{entities} $A_e$, \textit{relationships} $A_r$, and \textit{attributes} $A_a$. A \textit{compound} $C$ is defined as a primitive composition of multiple atoms, which correspond to connections between scene graph nodes. For visual concepts, there are two forms of primitive compositions and therefore two types of compounds: the semantic attachment of attribute to entities (``black dog”) $C_{ae}$, and the attachment of two entities via a relationship (``man hugs child”) $C_{ere}$. 

The composition of these compounds form subgraphs $S$, which can readily be translated to natural language captions $T$. Conversely, captions $T$ composed of visual concepts can be parsed to become scene graphs $S$; such captions are often paired with images $I$ in training and evaluation datasets $\mathcal{D}$. We therefore represent such datasets as image-caption pairs $\{(I, T)\}$ or image-scene-graph pairs $\{(I, S)\}$ interchangeably.

\sunnie{TODO: add a transition sentence}
\citet{hupkes2020} proposes to test compositionality from five aspects: systematicity, productivity, substitutivity, localism and overgeneralisation. Out of these five aspects, our work primarily considers the first two: systematicity and productivity. We adapt and instantiate them to evaluate vision-language models' representations.

\subsection{Systematicity}
% \rak{We need to be more specific in these sections by what we mean when we say something is unseen or seen. Let's start using some mathematical notation for atoms, compositions, training sets, etc. Then we can use those notations to explain when an atom is unseen versus when a composition is unseen.}
% FYI: defining $\D$ as $\mathcal{D}$
Systematicity evaluates a model’s ability to systematically recombine seen atoms. Concretely, we measure a model's systematicity by determining what atoms and compounds have been seen during its training, splitting a given evaluation dataset according to the extent that a model has seen each text, and comparing the model's performance across these different compositional splits. We use $\mathrm{Seen(A, D)}$ to denote if an atom is seen in a dataset $\D$,  namely $\exists (I, S) \in \mathcal{D}: A \in S$, and $\mathrm{Seen(C, D)}$ to denote if a compound is seen in a dataset $\D$,  namely $\exists (I, S) \in \mathcal{D}: C \subseteq S$. 
% In the evaluation set of a model, an atom $A$ is considered \textit{seen} if it has appeared in any caption in this model's training set (that is, if $\exists (I, S) \in \mathcal{D}_{train}: A \in S$) and \textit{unseen} otherwise. Similarly, a compound $C$ is \textit{seen} if it is seen as a part of any caption in $\mathcal{D}_{train}$ (that is, if $\exists (I, T) \in \mathcal{D}_{train}: C \subseteq T$) and \textit{unseen} otherwise.

We then define three compositional splits of the evaluation dataset: Seen Compounds, Unseen Compounds and Unseen Atoms. Seen Compounds refers to the subset of the evaluation dataset in which all compounds of all texts (and thus all atoms too) have been seen in the training dataset, \ie $\D^{ret}_{SC}  = \{(I, S) \in \D_{eval} \,|\, \forall C \subseteq S: \mathrm{Seen}(C, \D_{train}) \}$. Unseen Compounds are the split where all atoms have been seen and where there exist compounds that have NOT appeared in the training set  \ie $\D^{ret}_{UC} = \{(I, S) \in \D_{eval} \,|\, (\forall A \in S: \mathrm{Seen}(A, \D_{train}) \land (\exists C \subseteq S: \neg \mathrm{Seen}(C, \D_{train})) \}$. Unseen Atoms refer to the examples which contain some atoms that have never been seen during training, \ie $\D^{ret}_{UA} = \{(I, S) \in \D_{eval} \,|\, \exists A \in S: \neg \mathrm{Seen}(A, \D_{train})\ \}$.

\subsection{Productivity} A vision-language model that exhibits \textit{productive} compositional behavior comprehends a caption for a given image regardless of that scene's complexity. Since a scene is infinitely parseable in theory, scene complexity is proxied by the complexity of a caption derived from the scene, which we define to be the number of atoms it contains. A productive V-L model should thus ground a caption correctly to its corresponding image, regardless of the number of atoms it must parse in the caption. Accordingly, we probe for productivity in a dataset of captions of increasing atomic complexity.

\subsection{Compositional evaluation via retrieval}
\input{figures/systematicity_figure}
We formulate our compositionality evaluation under the framework of zero-shot image-to-text and text-to-image retrieval so that we probe the representation space as directly as possible. Theoretically, any existing image-text datasets can be used as such retrieval sets for evaluation. However, one limitation of using only existing image-text pairs in the retrieval set is that the data can be noisy: for an image query, the texts of other images in the retrieval set can be weak negatives or unintended positives. A model can perform well because of the abundance of weak negatives or perform poorly due to unintended positives. This means that a model's retrieval performance doesn't necessarily reflect anything about its compositionalty. Therefore, we explicitly introduce hard negatives to our retrieval sets so that high retrieval performance relies on compositional visual and textual representations.

For a given ground truth caption of an image, a hard negative is a caption that does not faithfully represent the corresponding image, and differs by the ground truth caption a minimal atomic shift. By erring in a single, granular syntactic or semantic fashion, hard negatives allow for variations in retrieval performance to be attributable to a specific failure mode of a model's compositional comprehension. 
 
% \jerry{Both experiments cover negative generation, and it's a crucial part of what makes this work hard. So I think it should be discussed here at a high level. Here's my blurb about hard negatives:}



==> old/03_compositionality_v2.tex <==


%=====================
% PRODUCTIVITY FIGURE
\input{figures/productivity_figure}
%=====================

\section{Compositional evaluation}

Though the \textit{principle} of compositionality is well-defined, we echo the warning of Hupkes \textit{et al.}~\cite{hupkes2020compositionality} that this principle is formally vacuous if the syntax and semantics of the composed language are not established. Additionally, once a compositional language is established, it is necessary to define what behaviors to expect from a model that achieves comprehension of said language, as well as how to empirically measure those behaviors. Therefore, we first define the language underlying our compositional evaluation (Section~\ref{sec:language}); describe \textit{what} aspects of compositionality we evaluate (Sections~\ref{sec:systematicity},~\ref{sec:prodictivity}); and explain \textit{how} we evaluate them via retrieval (Section~\ref{sec:retrieval}). 

\subsection{Compositional language of visual concepts}
\label{sec:language}
% We are primarily concerned with a language of visual concepts, particularly as expressed by the images and corresponding scene graphs of Visual Genome. Accordingly, an \textit{atom} is defined a particular node in a Visual Genome scene graph. These are subdivided into \textit{objects}, \textit{relationships}, and \textit{attributes}. The compositional functions correspond to connection between scene graph nodes in Visual Genome: namely, the semantic attachment of attribute to objects (``black dog”), and the attachment of two objects via a relationship (``man hugs child”). On top of this, our experiments also incorporate the attachment of a negation term onto any atom (``not black").
To evaluate vision-language models specifically, we find that a compositional language consisting of \textit{scene graph} visual concepts is an appropriate foundation~\cite{krishnavisualgenome}. Accordingly, an \textit{atom} $A$ is defined as a singular visual concept, corresponding to a single scene graph node. Atoms are subtyped into \textit{objects} $A_o$, \textit{relationships} $A_r$, and \textit{attributes} $A_a$. A \textit{compound} $C$ is defined as a primitive composition of multiple atoms, which corresponds to connections between scene graph nodes. For visual concepts, there are two forms of primitive compositions and therefore two types of compounds: the semantic attachment of attribute to objects (``black dog”) $C_{ao}$, and the attachment of two objects via a relationship (``man hugs child”) $C_{oro}$.

The composition of these compounds form subgraphs $S$, which can be translated to natural language captions $T$. Conversely, captions $T$ composed of visual concepts can be parsed to become scene graphs $S$; such captions are often paired with images $I$ in training and evaluation datasets $\mathcal{D}$. We therefore represent such datasets as image-caption pairs $\{(I, T)\}$ or image-scene-graph pairs $\{(I, S)\}$ interchangeably. This extensible language is capable of capturing a number of linguistic phenomena identified in existing literature~\cite{suhr-etal-2019-corpus,parcalabescu-etal-2022-valse}, including the existence of concepts (``a photo with \textit{flowers}''), spatial relationships (``a grill \textit{on the left of} a staircase''), action relationships (``a person \textit{throwing} a frisbee''),  presupposition (``The bird is perched on a \textit{nest}''), prepositional attachment (``A bird with \textit{green} wings''), and negation (``There are \textit{no} trucks on the road'').


%=====================
% TABLE OF HARD NEGATIVES
%\input{tables/productivity_error_modes.tex} 
%=====================


%=====================
% DATASET SIZES
\input{tables/dataset_summary}
%=====================

\subsection{Systematicity}
\label{sec:systematicity}

With our compositional language in place, we now define two dimensions of compositionality—systematicity and productivity—which we adapt to vision-language representations.
\textit{Systematicity} evaluates a model’s ability to systematically recombine seen atoms in compounds. Concretely, 
let $\textsc{Seen}(A, D)$ denote if an atom is seen in a training dataset $\D$,  namely $\exists (I, S) \in \D: A \in S$, and $\textsc{Seen}(C, D)$ denote if a compound is seen in a dataset $\D$,  namely $\exists (I, S) \in \D: C \subseteq S$. To evaluate systematicity, we define three compositional splits of an evaluation dataset: Seen Compounds ($\textsc{SC}$), Unseen Compounds ($\textsc{UC}$) and Unseen Atoms ($\textsc{UA}$).
%we measure a model's systematicity by creating three splits in an evaluation dataset: seen compositions, unseen compositions, and unseen atoms.
% first identifying what atoms and compounds have been seen during its training, splitting a given evaluation dataset according to the extent that a model has seen each text, and comparing the model's performance across these different compositional splits.
% In the evaluation set of a model, an atom $A$ is considered \textit{seen} if it has appeared in any caption in this model's training set (that is, if $\exists (I, S) \in \mathcal{D}_{train}: A \in S$) and \textit{unseen} otherwise. Similarly, a compound $C$ is \textit{seen} if it is seen as a part of any caption in $\mathcal{D}_{train}$ (that is, if $\exists (I, T) \in \mathcal{D}_{train}: C \subseteq T$) and \textit{unseen} otherwise.
\begin{itemize}
\item $\textsc{SC}$ refers to the subset of examples in which all compounds of all texts (and thus all atoms too) have appeared in the training dataset, \ie $\D_{\textsc{SC}}  = \{(I, S) \in \D_{test} \,|\, \forall C \subseteq S: \textsc{Seen}(C, \D_{train}) \}$. 
\item $\textsc{UC}$ is the split where all atoms have been seen and where there exists compounds that have NOT appeared in the training set  \ie $\D_{UC} = \{(I, S) \in \D_{test} \,|\, (\forall A \in S: \textsc{Seen}(A, \D_{train}) \land (\exists C \subseteq S: \neg \mathrm{Seen}(C, \D_{train})) \}$. 
\item $\textsc{UA}$ refer to the examples which contain at least one atom that has NOT been seen during training, \ie $\D_{UA} = \{(I, S) \in \D_{test} \,|\, \exists A \in S: \neg \textsc{Seen}(A, \D_{train})\ \}$.
\end{itemize}

\subsection{Productivity} 
\label{sec:prodictivity}
Productivity refers to a capacity to comprehend an unbounded set of expressions. Assuming that the set of atoms in any dataset is finite, a reasonable substitute for testing unbounded comprehension is testing comprehension over increasingly complex scenes. Therefore, a vision-language model that exhibits \textit{productive} compositional behavior comprehends a scene regardless of that scene's complexity, which we define as the number of atoms the scene graph $S$ contains, \ie $|S|$. 
%In our evaluation regime, a model's scene comprehension is probed by evaluating its retrieval performance within an image-text corpus (Section \ref{sec:retrieval}), with each image-text pair corresponding to a scene. 
Now, an image $I$ does not have a notion of complexity, since it is theoretically infinitely describable; on the other hand, captions $C$ do have a well-defined notion of complexity, which is the number of atoms in its corresponding scene graph $|S_T|$. Therefore, given an image, a productive model should be able to match the image to the correct corresponding caption, regardless of the number of atoms contained in the caption. 

To evaluate productivity, we define a range $n$ (in our case, $n = 4, 5, \dots, 12$) of productivity complexity. 
% we take an evaluation dataset of images and scene graphs and use the scene graphs to systematically generate captions of complexity $n$ over a sufficiently large range of $n$ (in our case, $n = 4, 5, \dots, 12$). 
We need splits of the evaluation dataset based on this complexity, where image-text pairs in a given split have a fixed complexity $n$, and evaluate a model's performance over each split.


\subsection{Compositional evaluation via retrieval}
\label{sec:retrieval}
We evaluate compositional reasoning using zero-shot image-to-text and text-to-image retrieval. This formulation probes the representation space as directly as possible and is already the most common evaluation method for vision-language foundation models~\cite{radford2021learning}. Theoretically, any existing image-text dataset can be used as such retrieval sets for evaluation. However, one challenging limitation in existing datasets renders the metrics evaluated on them inaccurate. Consider using an image query of a ``plant inside a yellow vase on top of a black television''. Retrieving unintended alternative positives, such as ``a black television'', is not necessarily incorrect. Similarly, if there are no other texts containing a ``plant'' and a ``television'' in the retrieval set, retrieving the correct text doesn't imply that the model understands the composition of atoms in the image. 
Ideally, to properly evaluate a model, the retrieval dataset should contain \textit{hard negatives} for every query. A hard negative is a caption that does not faithfully represent the corresponding image, and differs from the ground truth caption by some minimal atomic shift. A example hard negative for the query above is ``\textit{man} inside a yellow vase on top of a black television''. By erring in a single, granular syntactic or semantic fashion, hard negatives allow for variations in retrieval performance to be attributable to a specific failure mode of a model's compositional comprehension (see Appendix). 
We address this need for a new benchmark dataset to evaluate systematicity and productivity of vision-language models.

%limitation of using only existing image-text pairs in the retrieval set is that the data can be noisy: for an image query, the texts of other images in the retrieval set can be weak negatives or unintended positives. A model can perform well because of the abundance of weak negatives or perform poorly due to unintended positives. This means that a model's retrieval performance doesn't necessarily reflect anything about its compositionality. Therefore, we explicitly introduce hard negatives to our retrieval sets so that high retrieval performance relies on compositional visual and textual representations.

% For a given ground truth caption of an image, a hard negative is a caption that does not faithfully represent the corresponding image, and differs by the ground truth caption by a minimal atomic shift. By erring in a single, granular syntactic or semantic fashion, hard negatives allow for variations in retrieval performance to be attributable to a specific failure mode of a model's compositional comprehension. 


==> old/04_methods_v1.tex <==
\section{\name: a large-scale benchmark for vision-language compositionality}
\input{figures/productivity_figure}
% \omer{Open with a sentence-long summary of the section}
% \textit{}
There are several challenges to creating image-text retrieval datasets that evaluate compositional systematicity and productivity. For the systematicity, the primary challenge lies in parsing the training dataset for seen atoms and compounds in order to split the data into the three compositional splits accordingly. For productivity, the major challenges are generating image-text pairs across different text complexities as the retrieval sets. For both datasets, it is crucial to enumerate different types of hard negatives, to name the error mode each negative probes, and to design an automated hard negative generator which ensures the incorrectness of the negatives it generates. Additionally, we also need to filter out low-quality data to avoid the effect of confounding factors such as image resolution and atom count on models' retrieval performance. We detail our methods for tackling these challenges for future efforts attempting to create similar benchmarks for other training datasets.

% To test models' compositional understanding explicitly and purely, we perform two additional important steps in our creation of both datasets: filtering out low-quality data and augmenting the retrieval sets with hard negative captions. We filter out low-quality data to avoid the effect of confounding factors such as image resolution and atom count on models' retrieval performance. Furthermore, we also introduce methods to generate different types of hard negatives that expose models' failure modes in compositional understanding. We detail our methods for tackling these challenges in creating the evaluation datasets for compositional systematicity and productivity.  

\subsection{Systematicity dataset creation}
We develop a method to repurpose and augment existing datasets for evaluating the systematicity of any vision-language model’s representations where the model's training set is known and accessible. This method can be applied on any image-text dataset that isn't included in the training set of this model.  

\noindent\textbf{Parse training texts for seen atoms and compounds and split evaluation data}
First, we parse the texts in the training set to obtain seen atoms and compounds with the Stanford Scene Graph Parser. Since the parser only parses for entities and relationships, we further extract any attributes from the entities via spaCy's natural language processing parser by checking if the token's part-of-speech tagging is ADJ. After we obtain  all the seen atoms and compounds through text parsing, we divide all the image-text pairs in the evaluation set into the three compositional splits based on the presence of unseen atoms and/or compounds in the texts. 


\noindent\textbf{Filter evaluation data}
\label{sec:filter}
We perform the following filtering steps on the image-text pairs in all splits: we only keep region crops which have an area greater than or equal to 40K pixels, occupy at least 10\% of the whole image, and whose width-to-height ratio is between 0.5 and 2.0. We only include texts which have at least two atoms and one compound and the first of all examples with duplicated texts. 

\noindent\textbf{Generate hard negatives} 
In our systematicity evaluation dataset, we introduce two types of hard negatives HN1 and HN2. These hard negatives are generated by binding correct atoms in the caption with atomic foils, introducing wrong compounds that don't appear in the query image. HN1 introduces one incorrect compound by replacing one of the atoms with an atomic foil. HN2 concatenates two wrong compounds, where each contains an atomic foil. We only generate negatives for one-compound examples for systematicity evaluation, as productivity covers complex captions with more atoms.  Table x presents these negative examples. 

% We construct aset with one-compound examples and their negatives.  In each retrieval set, the query is an image and the target set contains one groundtruth caption and ten negative captions. The nine negative captions include two weak negatives, three HN2s and four HN1s. We only perform image-to-text retrieval on this contrast set, since text-to-image retrieval would require negative images that are substantially harder to synthesize. 



\subsection{Productivity dataset creation}
Recall that a vision-language model that exhibits productive compositional behavior is able to comprehend scenes described with a high quantity of atoms. 

In this section, we describe how image to text retrieval sets are created to assess model productivity. First, ground truth (GT) captions are generated via random walks of Visual Genome scene graphs. Second, 3 types of hard negatives are generated for these ground truth captions. Finally, these are assembled into retrieval sets $R_{n, i}$, with GT captions of complexity $n$ and hard negatives of type $i$. A separate evaluation is performed for each HN type $i$, in which retrieval performance on the sets $R_{n, i}$ is calculated and compared across caption complexities $n$.

\noindent\textbf{Caption Generation}
Unlike the systematicity experiment, we do not parse an evaluation image-\textit{caption} dataset because we cannot control for caption complexity within it. We instead begin with an image-\textit{scene graph} dataset to systematically generate captions of varied complexities. 

For a particular scene graph, our strategy for generating captions of a fixed complexity $n$ consists of two steps. First, we perform a random walk through the scene graph to generate a subgraph. The walk initializes a scene graph at a random object and, at any step, adds a compound to that graph. If a relationship ($C_{ere}$) is added, the walk continues from the newly added object; otherwise, the walk is continued from the same object. If the entire connected component is exhausted, another object is selected at random from a different connected component. This process ends when $n$ atoms are added to the subgraph.

For each scene graph and complexity $n$, we repeatedly perform $n$-length random walks to generate $k = 4$ subgraphs. Each subgraph corresponds to a specific crop of the image, determined by the union of the bounding box of every atom in the subgraph. We apply the same region crop filters as outlined in Section \ref{sec:filter} to ensure acceptable image sizes and dimensions. Additionally, we ensure that subgraphs of the same complexity derived from the same image had bounding boxes which overlapped no more than 75\%. 

Next, we convert each subgraph to a caption using two different approaches. The first approach, used for complexities $n \leq 6$, iteratively strings all objects with attributes together (e.g.\ \texttt{boy + (tall,blue) => tall and blue boy}) and then strings together these clauses via their relationships. (e.g.\ \texttt{boy=(tall,blue); grass=(green); (boy, on, grass) => tall and blue boy on green grass}) to generate the final caption. The second approach, used for $n \geq 7$, employs a few-shot prompt to GPT that requests a caption given a textual representation of the subgraph. This textual representation simply lists all the objects and relationships:
\texttt{"OBJECTS: bushes; flower; bench; woman. RELATIONS: bushes are behind a bench; bench behind woman"}. For each complexity $n$, 1 to 3 captions were manually written for 5 randomly sampled $n$-atom subgraphs; these captions are then used as examples in prompts for generating the remaining captions. 

\noindent\textbf{Generating Hard Negatives}
For productivity, we explore 3 hard negatives types (``HN types"), each attributed with a hypothesized model error mode. Table \ref{tab:proderrors} enumerates these HN types, along with $h_i$, the number of hard negatives of type $i$ we generate per ground truth caption.

\input{tables/productivity_error_modes.tex}

For each HN type, the procedure to generate a hard negative for a given caption are as follows:

\paragraph{E/HN1: Atomic hard negatives}
    Our first hypothesized error mode is that, as a caption's complexity increases, a model may begin to ignore the caption's individual details. Accordingly, atomic hard negatives probe a model's capacity to recognize individual details in a caption. 
    
    To generate an atomic hard negative given a ground truth caption, an atom is randomly selected from the caption and replaced with an atom which negates the caption. Since annotations are non-exhaustive, this replacement must be done carefully. For example, if a dog is white and furry, but only ``white'' is annotated, replacing the atom `white" in ``white dog" with ``furry" would result in a correct caption. To minimize errors, we employ Wordnet, which provides a hierarchical semantic relationship between atoms, to ensure replacement atoms are mutually exclusive to the original atom. A replacement atom must either by an explicit antonym of the original atom when available (``\textit{black} dog") or a ``cousin atom,'' which means they share the same grand-hypernym (``\textit{pink} dog").
    
\paragraph{E/HN2: Swapping hard negatives}
    \jerry{Gotta shout out winoground here}
    Swapping hard negatives probe a model's capacity to . To generate an swapping hard negative given a ground truth caption, two atoms are swapped and the caption is regenerated. The following pairs of atoms could be swapped to create a hard negative:
    \begin{itemize}
        \item The subject and object of an \textit{asymmetric} relationship -- this is verified by determining whether there was a big shift in perplexity \jerry{(over what?)} upon changing the caption.
        \item Two attributes attached to distinct objects, such that one attribute is not present for the other object in the scene graph and vice versa.
        \item Two random, distinct objects not connected by a relationship, unless their relationships are identical.
    \end{itemize}
    Additionally, some hard negatives are permutations rather than a swapped pair:
    \begin{itemize}
        \item One attribute can be transferred to another object, so long as that attribute doesn't apply to the new object.
        \item For low complexities ($n = 4$), any permutation of atoms of the same type are allowed. For example: (``there is a dog on the bed and also a nightstand" -> ``there is a nightstand on the dog and also a bed")
    \end{itemize}
    
\paragraph{E/HN3: Negating hard negatives}
    Negating hard negatives probe a model's capacity to recognize the ``not" modifier. To generate a negating hard negative given a ground truth caption, either
    \begin{itemize}
        \item Negate the entire caption by appending “this image does not contain” in a grammatically correct fashion.
        \item Pick an attribute $A$ replace it with the clause "that is not $A$" in a grammatically correct fashion.
        \item Pick a relationship $R$ and replace it with (”is not $R$") in a grammatically correct fashion
        \item Pick an object and its corresponding attributes ($C$) and replace it with (``no $C$", or ``object that is not $C$")
    \end{itemize}
    For relationships and attributes connected to object $o$, we verify that negating the attribute does not transform the object to another existing object $o'$ which may share all but one of the same relationships and attributes.


\noindent\textbf{Retrieval dataset construction}
\jerry{Summarize some important points about the retrieval set here?}
For each HN type $i \in \{1, 2, 3\}$ and complexity $n \in \{4, 5, \dots, 12\}$, we construct $R_{n, i}$, which contains $N = 5000$ images paired 1-to-1 with ground truth captions; this constitutes a total of $N_{tot} = 45000$ captions generated. 

In $R_{n, i}$, each ground truth caption has $h_i$ corresponding hard negatives, for a total of $N(h_i + 1)$ captions per retrieval set. Then, for a fixed $i$, we evaluate retrieval metrics for $R_{n, i}$ across all values of $n$. 

\subsection{Implementation details}
In this paper, we instantiate this method to create systematicity and productivity evaluation datasets with the Visual Genome scene graphs. For the systematicity dataset, we use the region crops in Visual Genome as images and spelling-corrected descriptions as texts in our retrieval sets. \sunnie{For productivity, anything to say here? @Jerry}
In total, we have x and y image-text pairs as well as x and y negative captions in the systematicity and productivity evaluation datasets. 

\subsection{Data verification}
We verified the validity of a $?\%$ sample of our ground truth captions. This was done manually through 2 pairs of human annotators. Each pair was given the same set of captions to label; for each caption, they were prompted with the question "Is this a faithful caption for the image?," and answered either yes or no.

\jerry{STATS HERE}

==> old/04_methods_v2.tex <==
\section{\name: a large-scale benchmark for vision-language compositionality}
\input{figures/productivity_figure}
% \omer{Open with a sentence-long summary of the section}
% \textit{}
There are several challenges to creating image-text retrieval datasets that evaluate compositional systematicity and productivity. For systematicity, the primary challenge lies in parsing the training dataset for seen atoms and compounds in order to split the data into the three compositional splits accordingly. For productivity, the major challenges are generating image-text pairs across different text complexities as the retrieval sets. For both datasets, it is crucial to enumerate different types of hard negatives, to name the error mode each negative probes, and to design an automated hard negative generator which ensures the incorrectness of the negatives it generates. Additionally, we also need to filter out low-quality data to avoid the effect of confounding factors such as image resolution and atom count on models' retrieval performance. We detail our methods for tackling these challenges for future efforts attempting to create similar benchmarks for other training datasets.

% To test models' compositional understanding explicitly and purely, we perform two additional important steps in our creation of both datasets: filtering out low-quality data and augmenting the retrieval sets with hard negative captions. We filter out low-quality data to avoid the effect of confounding factors such as image resolution and atom count on models' retrieval performance. Furthermore, we also introduce methods to generate different types of hard negatives that expose models' failure modes in compositional understanding. We detail our methods for tackling these challenges in creating the evaluation datasets for compositional systematicity and productivity.  

\subsection{Systematicity dataset creation}
To create the three systematicity splits—seen compounds, unseen compounds, unseen atoms—we parse a given training dataset $\D$ into its constituent atoms and compounds, filter low-quality data, and generate hard negatives.

% We develop a method to repurpose and augment existing datasets for evaluating the systematicity of any vision-language model’s representations where the model's training set is known and accessible. This method can be applied on any image-text dataset that isn't included in the training set of this model.  

\noindent\textbf{Parsing a dataset into atoms and compounds}
Since we utilize the scene graph representation as our compositional language, we parse texts in the training set into their corresponding scene graphs with objects, attributes and relationships. we use the Stanford Scene Graph Parser~\cite{schuster2015generating}. Since the parser only parses for objects and relationships, we further extract the attributes from the text via spaCy's natural language processing parser by identifying adjective part-of-speech tags. These objects, attributes, and relationships constitute our seen atoms and compounds. Similarly, we parse a given evaluation set and  divide all the image-text pairs into the three compositional splits based on the presence of unseen atoms and/or compounds in the parsed training set.


\noindent\textbf{Filter evaluation data}
\label{sec:filter}
We perform the following filtering steps on the image-text pairs in all splits: we only keep region crops which have an area greater than or equal to 40K pixels, occupy at least 10\% of the whole image, and whose width-to-height ratio is between 0.5 and 2.0. We only include texts which have at least two atoms and one compound and the first of all examples with duplicated texts. 

\noindent\textbf{Generate hard negatives} 
In our systematicity evaluation dataset, we introduce two types of hard negatives HN1 and HN2. These hard negatives are generated by binding correct atoms in the caption with atomic foils, introducing wrong compounds that don't appear in the query image. HN1 introduces one incorrect compound by replacing one of the atoms with an atomic foil. HN2 concatenates two wrong compounds, where each contains an atomic foil. We only generate negatives for one-compound examples for systematicity evaluation, as productivity covers complex captions with more atoms.  Table x presents these negative examples. 

% We construct aset with one-compound examples and their negatives.  In each retrieval set, the query is an image and the target set contains one groundtruth caption and ten negative captions. The nine negative captions include two weak negatives, three HN2s and four HN1s. We only perform image-to-text retrieval on this contrast set, since text-to-image retrieval would require negative images that are substantially harder to synthesize. 



\subsection{Productivity dataset creation}
Recall that a vision-language model that exhibits productive compositional behavior is able to comprehend scenes described with a high quantity of atoms. In this section, we describe how image to text retrieval sets are created to assess model productivity: generating ground truth captions, generating hard negatives, and splitting captions into the appropriate retrieval sets.
% First, ground truth (GT) captions are generated via random walks of Visual Genome scene graphs. Second, 3 types of hard negatives are generated for these ground truth captions. Finally, these are assembled into retrieval sets $R_{n, i}$, with GT captions of complexity $n$ and hard negatives of type $i$. A separate evaluation is performed for each HN type $i$, in which retrieval performance on the sets $R_{n, i}$ is calculated and compared across caption complexities $n$.

\noindent\textbf{Caption Generation}
Unlike the systematicity experiment, we do not parse an evaluation image-\textit{caption} dataset because we cannot control for caption complexity within it. We instead begin with an image-\textit{scene graph} dataset to systematically generate captions of varied complexities. 

For a particular scene graph, our strategy for generating captions of a fixed complexity $n$ consists of two steps. First, we perform a random walk through the scene graph to generate a subgraph. 
% For each scene graph and complexity $n$, we repeatedly perform $n$-length random walks.
% to generate $k = 4$ subgraphs. 
Each subgraph corresponds to a specific crop of the image, determined by the union of the bounding boxes of subgraph atoms. We apply the same region crop filters as outlined in Section \ref{sec:filter} to ensure acceptable image sizes and dimensions. 
Additionally, we ensure that subgraphs of the same complexity derived from the same image had IOU boxes with IOUs of no more than 75\%. 

Next, we caption each subgraph. For simple subgraphs of complexity $n=4$, we produce captions by stringing together subjects, relations, and objects (e.g.\ \texttt{boy=(tall,blue); grass=(green); (boy, on, grass) => tall and blue boy on green grass}). Any disconnected atoms are appended with the prefix ``and a''. 
For all other subgraphs ($n=5, \cdots, 12$), we leverage GPT-3 (text-davinci-002) to generate captions based on a text description of the scene graph, which lists all objects and relationships. 
We prompted GPT-3 using 5 manually written captions per complexity. 
To ensure captions are as complex as their original subgraphs, we filtered out captions which omitted objects from the subgraph.
To verify caption quality, we ran manual verification in Section \ref{sec:verification}, and we provide more details about prompting strategy in the Appendix.

\noindent\textbf{Generating Hard Negatives}
For productivity, we explore 3 hard negatives types (``HN types"), each attributed with a hypothesized model error mode. Table \ref{tab:proderrors} enumerates these HN types, along with $h_i$, the number of hard negatives of type $i$ we generate per ground truth caption.

\input{tables/productivity_error_modes.tex}

Our first hypothesized error mode is that, as a caption's complexity increases, a model may begin to ignore the caption's individual details. Accordingly, an \textit{atomic hard negative} (AHN) probes a model's capacity to recognize individual details by randomly selected an atom from the caption and replaced with an atom which negates the caption. Since annotations are non-exhaustive, this replacement must be done carefully. For example, if a dog is white and furry, but only ``white'' is annotated, replacing the atom `white" in ``white dog" with ``furry" would result in a correct caption. To minimize errors, we employ Wordnet, which provides a hierarchical semantic relationship between atoms, to ensure replacement atoms are mutually exclusive to the original atom. A replacement atom must either by an explicit antonym of the original atom when available (``\textit{black} dog") or a ``cousin atom,'' which means they share the same grand-hypernym (``\textit{pink} dog").

Our second hypothesized error mode is that, as a caption's complexity increases, a model may begin to interpret a caption as a ``bag of words," ignoring synctatic connections built out of word order. Accordingly, a \textit{swap hard negative} (SHN) permutes atoms in the caption such that the new caption contains the same set of atoms but is an incorrect description. This hard negative maps to the work of Winoground ~\cite{thrush2022winoground}, but in the context of varying caption complexity.
The two atoms are selected such that they belong to the same subcategory and that their swapping negates the caption -- see Section \ref{sec:swap_atoms} for specific examples of swappable atoms.
  
Our third hypothesized error mode is that, as a caption's complexity increases, a model may begin to lose comprehension of negations. Accordingly, \textit{negation hard negatives} probe a model's capacity to recognize the ``not" modifier. These are generated either by negating the entire caption or a specific atom. We inspect each caption's original full scene graph to verify that the negation results in a false caption.
    

\noindent\textbf{Retrieval dataset construction}
For each HN type $i \in \{1, 2, 3\}$ and complexity $n \in \{4, 5, \dots, 12\}$, we construct $R_{n, i}$, which contains $N = 5000$ images paired 1-to-1 with ground truth captions; this constitutes a total of $N_{tot} = 45000$ captions generated. 

In $R_{n, i}$, each ground truth caption has $h_i$ corresponding hard negatives, for a total of $N(h_i + 1)$ captions per retrieval set. Then, for a fixed $i$, we evaluate retrieval metrics for $R_{n, i}$ across all values of $n$. 

\subsection{Implementation details}
\irena{move this to the top of section 4? this seems like a summary of CREPE}
In this paper, we instantiate this method to create systematicity and productivity evaluation datasets with the Visual Genome scene graphs. For the systematicity dataset, we use the region crops in Visual Genome as images and spelling-corrected descriptions as texts in our retrieval sets. \sunnie{For productivity, anything to say here? @Jerry}
In total, we have $385K$, $385K$ and
$373K$ image-text pairs and $237K$, $210K$ and $178K$ hard negative captions for evaluating models trained on CC12M, YFCC15M and LAION400M across the compositional splits. For productivity evaluation, our dataset contains more than $17K$ image-text pairs across nine complexities and and $246K$ hard negative captions of three different types. 

\subsection{Data verification} \label{sec:verification}
To measure data quality in \name~, we manually verified samples of ground-truth captions generated by GPT-3 in the productivity dataset, as well as hard negative samples in both the systematicity and productivity datasets.

We sampled 2\% of productivity ground truth captions generated by GPT-3, \irena{?\%} of productivity hard negatives, and \irena{?\%} of systematicity hard negatives for verification. 
For ground truth captions, annotators verified caption faithfulness to the image, while for hard negatives, annotators verified that strings actually do make factually incorrect statements about the image (\ie are genuine negatives).
We divided each set between 2-4 annotators and measure both caption / negative quality and intra-annotator agreement.

87.9\% of sampled ground truth captions generated by GPT-3 from the productivity dataset were rated as faithful to the image, with average pairwise annotator agreement of 88.8\%. 
78.1\% of productivity hard negatives and 77.6\% of systematicity hard negatives were rated as genuine negatives, with pairwise annotator agreements of 66.3\% and 67.1\% respectively.

\irena{include accuracies per complexity and across hard negative types}

==> old/04_methods_v3.tex <==


%=====================
% SYSTEMATICITY HARD NEGATIVES
\input{tables/systematicity_hard_negs}
%=====================


\section{\nameemoji: a large-scale benchmark for vision-language compositionality}

There are several challenges to creating image-text retrieval datasets that evaluate compositional systematicity and productivity. For systematicity, the primary challenge lies in parsing the training dataset for seen atoms and compounds in order to split the data into the three according compositional splits. For productivity, the major challenge is generating image-text pairs across different text complexities for the retrieval sets. For both datasets, it is crucial to enumerate different types of hard negatives, and to design an automated hard negative generator which ensures the incorrectness of the negatives it generates. 
% Additionally, it is crucial to filter out low-quality data to avoid the effect of confounding factors such as image resolution and atom count on models' retrieval performance. 
We detail our methods for tackling these challenges for future efforts that attempt to create similar benchmarks for other training datasets. 



\subsection{Creating systematicity datasets}
To create the three systematicity splits—$\textsc{SC}$, $\textsc{SA}$, $\textsc{UA}$—we parse a given training dataset $\D$ into its constituent atoms and compounds, filter low-quality data, and generate hard negatives (Figure~\ref{fig:systematicity}).

% We develop a method to repurpose and augment existing datasets for evaluating the systematicity of any vision-language model’s representations where the model's training set is known and accessible. This method can be applied on any image-text dataset that isn't included in the training set of this model.  

\noindent\textbf{Parsing a dataset into atoms and compounds}
Since we utilize the scene graph representation as our compositional language, we use the Stanford Scene Graph Parser~\cite{schuster2015generating} to parse texts in $\D_{train}$ into their corresponding scene graphs with objects, attributes and relationships. Since the parser only parses for objects and relationships, we further extract the attributes from the text via spaCy's natural language processing parser by identifying adjective part-of-speech tags. These connected objects, attributes, and relationships constitute our seen atoms and compounds. Similarly, we parse a given $\D_{test}$ and  divide all the image-text pairs into the three compositional splits based on the presence of unseen atoms and/or compounds in the parsed training set.


\noindent\textbf{Filtering low-quality data}
We perform the following filtering steps on the image-text pairs in all splits: we only keep region crops which have an area greater than or equal to $40K$ pixels, occupy at least $10\%$ of the whole image, and whose width-to-height ratio is between $0.5$-$2.0$. We only include text which have at least $2$ atoms and $1$ compound and de-duplicate text using their corresponding scene graphs. 

\noindent\textbf{Generating hard negatives} 
We introduce two types of hard negatives: $\textsc{HN-Atom}$ and $\textsc{HN-Comp}$.
$\textsc{HN-Atom}$ replaces $A_a$, $A_o$, or $A_r$ in the text with an atomic foil. For example, for the caption ``a grill on top of the porch'', one $\textsc{HN-Atom}$ can be ``a grill \textit{underneath} the porch'', where the $A_r$ ``on top of'' is replaced by ``underneath''. Since captions and scene graphs are not exhaustive, this replacement must be done carefully. For example, if a dog is white and furry, but only ``white'' is annotated, replacing the atom ``white'' with ``furry'' would result in a correct caption. To minimize errors, we employ Wordnet to pick replacement atoms that are either antonyms (``\textit{black} dog'') or share the same grand-hypernym (``\textit{pink} dog") with respect to the original atom. 
% which provides a hierarchical semantic relationship between atoms. to ensure replacement atoms are mutually exclusive to the original atom. A replacement atom must either by an explicit antonym of the original atom when available (``\textit{black} dog") or a ``cousin atom,'' which means they share the same grand-hypernym (``\textit{pink} dog"). 

$\textsc{HN-Comp}$ concatenates two compound foils  where each contains an atomic foil. For instance, one $\textsc{HN-COMP}$ of the caption ``a pink car'' can be ``a \textit{blue} car and a pink \textit{toy}'', where ``blue'' and ``toy'' are the atomic foils in the two compounds foils ``blue car'' and ``pink toy''. We only generate negatives for one-compound examples for systematicity evaluation, as productivity covers complex captions with more atoms. 

% We construct aset with one-compound examples and their negatives.  In each retrieval set, the query is an image and the target set contains one groundtruth caption and ten negative captions. The nine negative captions include two weak negatives, three HN2s and four HN1s. We only perform image-to-text retrieval on this contrast set, since text-to-image retrieval would require negative images that are substantially harder to synthesize. 



\subsection{Creating productivity datasets}
For productivity, we first generate ground truth captions, generate hard negatives for each, and categorize each captions into the appropriate complexity (Figure~\ref{fig:productivity}).
% First, ground truth (GT) captions are generated via random walks of Visual Genome scene graphs. Second, 3 types of hard negatives are generated for these ground truth captions. Finally, these are assembled into retrieval sets $R_{n, i}$, with GT captions of complexity $n$ and hard negatives of type $i$. A separate evaluation is performed for each HN type $i$, in which retrieval performance on the sets $R_{n, i}$ is calculated and compared across caption complexities $n$.

\noindent\textbf{Generating captions}
To control exactly how many atoms occur in each caption, we systematically generate captions of different complexities for each image.
Given a scene graph, we perform a random walk of length $n$ through the scene graph to generate a subgraph.
Each subgraph corresponds to a specific region of the image, determined by the union of the bounding boxes of the subgraph atoms. We filter out low-quality regions using the same process as systematicity. 
% In order to avoid a scenario where this union captures objects not in the subgraph, we filter out patches that covered more than $75\%$ of the image. 
For simple subgraphs ($n=4$), we produce captions using handcrafted templates, which we describe in the Appendix. 
% (e.g.\ \texttt{boy=(tall,blue); grass=(green); (boy, on, grass) => tall and blue boy on green grass}). Any disconnected atoms are appended with the prefix ``and a''. 
For larger subgraphs ($n \geq 5$), we leverage GPT-3~\cite{brown2020language} (text-davinci-002) to generate captions based on a text description of the scene graph, which lists all objects and relationships. 
We prompt GPT-3 using 5 manually written captions per complexity and automatically filter captions where GPT-3 errs and omits atoms from the subgraph during generation (see Appendix).
% We manually verify this generation process (Section~\ref{sec:verification}).

%=====================
% SYSTEMATICITY WEAK NEGATIVES
\input{tables/systematicity_weak_negs}
%=====================

\noindent\textbf{Generating hard negatives}
For productivity, we employ three hard negatives types ($\textsc{HN-Atom}$ from systematicity, $\textsc{HN-Swap}$, and $\textsc{HN-Neg}$) corresponding to three hypothesized model error modes.
First, as a caption's complexity increases, a model may begin to ignore individual atoms. $\textsc{HN-Atom}$ randomly selects an atom from the caption and replaces it with an incorrect atom.
Second, as a caption's complexity increases, a model may treat captions as ``bags of words," ignoring syntactic connections built out of word order. A \textit{swap hard negative} ($\textsc{HN-Swap}$) accordingly permutes atoms of the same subtype in a caption. This hard negative is similar to Winoground~\cite{thrush2022winoground}, but in the context of varying caption complexity. The two atoms are selected such that they belong to the same subtypee and that their swapping negates the caption.
Finally, as a caption's complexity increases, a model may begin to lose comprehension of negations. A \textit{negation hard negative} ($\textsc{HN-Neg}$) either negates the entire caption or a specific atom.
%We inspect each caption's original full scene graph to verify that the negation results in a false caption.
    

% \noindent\textbf{Retrieval dataset construction}
% For each hard negative type $i$ and complexity $n$, we construct the test dataset $\D_{test}^{HN(n, i)}$, which contains $2K$ images paired with one ground truth captions and a set of $17K$ hard negatives.

% In $R_{n, i}$, each ground truth caption has $h_i$ corresponding hard negatives, for a total of $N(h_i + 1)$ captions per retrieval set. Then, for a fixed $i$, we evaluate retrieval metrics for $R_{n, i}$ across all values of $n$. 

\subsection{The final benchmark datasets}
We construct two forms of test datasets for productivity and systematicity. The first is $\D_{test}^{RAW}$, which contains ground truth image-text pairs, where the retrieval set contains negative captions from the raw original dataset. We perform both image-to-text and text-to-image retrieval within splits of $\D_{test}^{RAW}$. The second is $\D_{test}^{HN}$, which only contains image-text pairs with a retrieval set containing only the generated hard negatives. Here, we perform only image-to-text retrieval across splits, since we focus on generating hard negatives for text and not for images.
%; the query is an image, and the retrieval set contains just the corresponding ground truth caption and $h$ hard negatives, with $h$ varying based on dataset (see Appendix).
% ; to enable text-to-image retrieval, we leave the generation of ``hard negative images" to future work

When performing retrieval for systematicity, test datasets are split into $SC$, $UC$, and $UA$ for cross-comparison. For productivity, $\D_{test}^{RAW}$ is split by complexity $n$, and $\D_{test}^{HN}$ is further split by hard negative type $i$ for cross-comparison. 
% -- these are denoted as $\D_{test}^{HN(n, i)}$.


\subsection{Data verification} \label{sec:verification}
% We manually verify samples of ground-truth captions generated by GPT-3 in the productivity dataset, as well as hard negative samples in both the systematicity and productivity datasets.
To measure the data quality of \name{}, we randomly sample $2\%$ of productivity ground truth captions generated by GPT-3 and $1\%$ of the queries in the productivity and systematicity hard negatives set $\D_{test}^{HN}$ for manual verification. We divide each set between $4$ annotators and measure both caption / negative quality and intra-annotator agreement.
$87.9\%$ of sampled productivity ground truth captions generated by GPT-3 are rated as faithful to the image, with average pairwise annotator agreement of $88.8\%$. 
$78.1\%$ of productivity and $77.6\%$ of systematicity hard negatives were rated as genuine negatives (\ie made factually incorrect statements about the image), with pairwise annotator agreements of $66.3\%$ and $67.1\%$ respectively. 


==> old/05_experiments_v1.tex <==


\section{Experiments}
% \subsection{Task definition}
% \omer{One approach is to define the shared task on a high-level, mathematically. Reference the fact that we are using image-text retrieval as the task. Justify it. Task description should reference the use of weak and hard negatives, alongside why. Given that both tasks use retrieval metrics, it shouldn't hurt to define the main metrics here: mean/median GT rank, R@1/3/5 and the hard negative specific metrics.}

% \paragraph{Image to text retrieval} To evaluate model comprehension and probe the representation space as directly as possible, we construct retrieval datasets for all of our experiments. 
% To evaluate models' compositional comprehension and probe the representation space as directly as possible, we conduct zero-shot image-to-text and text-to-image retrieval evaluation of vision-language models on our datasets. 
We detail our experimental setup and then present our five main results in the following order: first, our systematicity experiments show that models perform similarly on Seen or Unseen Compounds; second, our evaluation on the retrieval sets with hard negatives demonstrates that models' Recall@1
performance drops more significantly up to 8\% when compositions are unseen; third, our productivity experiments show that mod-
els' performance decreases as the number
of atoms in the compositions increases; fourth, we find that a larger pretraining dataset size doesn't directly translate to better compositionality; finally, our results show that a larger model size could lead to small improvement in compositionality. 

\subsection{Experimental setup}
\textbf{Datasets} For both systematicity and productivity, we have two types of retrieval sets: $\D^{ret}_{RAW}$ which contains the raw image-text pairs, and $\D^{ret}_{HN}$ where image-text pairs are augmented with hard negative captions. For $\D^{ret}_{RAW}$, we perform both image-to-text and text-to-image retrieval, where the query is an image or text and the retrieval set consists of all texts or images in the $\D^{ret}_{RAW}$. 
For $\D^{ret}_{HN}$, we only perform image-to-text retrieval with generated hard negative captions in the retrieval set, as it is much more challenging to generate hard negative images than texts. In this case, the query is an image, and the retrieval set contains the groundtruth caption and $N$ hard negatives, with $N$ varying based on dataset (Table \ref{fig:prod_hard_negs}).

\textbf{Models} We evaluate seven vision-language models pretrained with the CLIP loss~\cite{radford2021learning} across three commonly used image-text datasets: Conceptual Captions 12M (CC-12M)~\cite{changpinyo2021conceptual}, a subset of the YFCC100M dataset (YFCC-15M)~\cite{thomee2016yfcc100m, radford2021learning} and LAION-400M~\cite{schuhmann2021laion}. These include two visual encoders, ResNet (RN)~\cite{he2016deep} and Vision Transformer (ViT)~\cite{dosovitskiy2021an}, of different sizes: RN50, RN101, ViT-B-16, ViT-B-16-plus-240, ViT-B-32 and ViT-L-14. Due to the computational challenge of training such models on large datasets, we use pretrained checkpoints provided by OpenCLIP repository~\cite{Ilharco_OpenCLIP_2021}.

\textbf{Metrics} We adopt the most commonly used metrics in retrieval-based studies, Recall@1, 3, 5 and Average Recall@K. For $\D^{ret}_{RAW}$, we primarily report the mean and standard deviation of Recall@1 across K-fold retrievals (where $K = \min(20, )$), as the data size varies across compositional splits and complexities. For $\D^{ret}_{HN}$, we report the mean Recall@1 and 3 values.
% where at each fold we \textit{resample from the set of feasible hard negatives for each ground truth caption for productivity and resample from the compositional split in systematicity.}

\subsection{Systematicity Evaluation}
\paragraph{Model Recall@1 decreases monotonically between systematicity splits.} This is the case for both $\D^{ret}_{HN}$ (Table \ref{tab:systematicity_hard_negs})and $\D^{ret}_{RAW}$ (Table \ref{tab:systematicity_weak_negs}) datasets for systematicity.  This drop is consistently smaller than $2\%$ for models trained on CC-12M and YFCC-15M, but pronounced for LAION-400M models. For instance on $\D^{ret}_{HN}$, LAION-400M models, with the exception of ViT-L-14, experience Recall@1 drops of approximately $5\%$ or higher, with the relative drop in performance from Seen all compounds (SC) values reaching $16.29\%$ for Vit-B-32. It is also important to note that while CC-12M and YFCC-15M models suffer small decreases between splits, they also greatly underperform LAION-400M models, meaning that this small decrease could be due to an overall poor performance rather than systematic generalization.
\input{figures/modelPerfvsRecall_syst.tex}


\subsection{Productivity Evaluation}
\paragraph{Models' performance decreases with complexity on HN-ATOM and HN-SWAP negatives.} 

\input{figures/produtivity_hard_negs_plot}

At small complexities such as $n=4$, we observe that model retrieval quality is well-above random chance  (Figure \ref{fig:prod_hard_negs}). However, as caption complexity increases, we observe a steady decrease in recall performance, nearing random chance for HN-ATOM and dipping below it for HN-SWAP negatives. While past work demonstrates that vision-language models struggle with atomic ~\cite{parcalabescu-etal-2022-valse, park-etal-2022-exposing} and swapping~\cite{thrush2022winoground, yuksekgonul2022and} foils, these two trends together demonstrate that models' ability to correctly identify ground-truth captions from foils is dependent on caption complexity as well, indicating difficulty with productivity. For HN-NEG foils, we do not observe a downward trend but find that models' performance is stable but poor, particularly for YFCC-15M, where Recall@1 is consistently below chance.



\include{figures/modelPerfvsRecall_prod.tex}

\subsection{Performance based on pretraining dataset}
We also compare retrieval ability, stratified by training dataset.
In the systematicity hard negatives experiment, we observe a clear gap in performance with stratifying across pretraining datasets, with LAION-400M models scoring best Recall @ 1 across the Seen Compounds and Unseen Compounds splits in Table \ref{tab:systematicity_hard_negs}. This gap decreases as we relax the evaluation metric, with Retrieval @ 5 being close across models trained on all datasets on both seen and unseen compounds splits. 
We also observe that the recall drop between the Seen Compounds and Unseen Compounds splits is \textit{steeper} for larger models trained on larger datasets; \ie while CC12M models only drop 2 percentage points in R@1 between the two splits, LAION models drop up to 8 percentage points between the Seen and Unseen splits.

In the systematicity weak negatives experiment (Table \ref{tab:systematicity_weak_negs}), we see a similar gap in Retrieval @ 1 between LAION-trained models (which are larger) and those trained on smaller datasets across both the image-to-text and text-to-image tasks.
We also observe larger drops on LAION-trained models when moving across the Seen Compounds, Unseen Compounds, and Unseen Atoms splits, with LAION models dropping as much as 13 percentage points between the Seen Compounds and Unseen Atoms experiments (ViT-L/14, text to image).


We display productivity experiment results, with separate lines for each pretraining dataset, in Figure \ref{fig:prod_hard_negs}.
Unlike in the systematicity experiments, we do not observe a clear advantage for larger pretraining datasets in this set of experiments.
When the hard negative type is atomic foils (Figure \ref{fig:prod_hard_negs}, left), we see similar performance for models trained on LAION400M and YFCC15M, with slightly worse performance overall for the model trained on CC12M. 
When the hard negative type is swaps (Figure \ref{fig:prod_hard_negs}, right), we see that all models (across all datasets) show similar retrieval perofrmance.
However, when the hard negative type is negations (Figure \ref{fig:prod_hard_negs}, center), we see variable performance based on pretraining dataset, with CC12M models (the smallest model and smallest dataset) outperforming LAION and YFCC models (larger models on larger datasets). \irena{TODO: are these negatives even sound?}
% We note that, in our results, there is no clear pattern suggesting that larger pretraining datasets (for which we also test larger models) lead to better retrieval performance.
% To isolate the influence of pretraining dataset from model architecture, we also compare group results on model type and compare across datasets in Figure \irena{I think Mona is working on this}.
% We see that \irena{todo once we have this analysis}.
% \irena{Discussion if the results are interesting.} We note that, in addition to differing in their sizes (12M, 15M, and 400M), these pretraining datasets also differ in their filtering protocol, with CC12M particularly optimizing for entity coverage~\cite{changpinyo2021conceptual}. 

% \irena{
%     the tricky part here is that the model sizes are conflated with the pretraining dataset. we have 
%     CC12M: RN50(23M), 
%     YFCC: RN50(23M), RN101 (44M),
%     LAION: ViT-B-16(86M), VitB16p(), VitB32(197M), Vitl14(307M)
% }


\subsection{Performance based on model size}
Lastly, we also compare retrieval ability across model sizes within a pretraining dataset (Figure \ref{fig:prodModelPerf}).
We examine two datasets for this section: YFCC15M (for which we evaluate a ResNet50 and a ResNet101) and LAION-400M (for which we evaluate ViT-B/16, Vit-B/16+, ViT-B/32, and ViT-L/14).

In figure \ref{fig:systModelPerf} (systematicity) we observe that larger models tend to have better retrieval abilities within LAION-400M, for which we have four models to compare. 
We also note that this ranking matches the relative rankings of zero-shot ImageNet accuracy reported by the OpenCLIP authors (where ViT-B/32 performs worst at 62.9\%, ViT-B/16 at 67.1\%, ViT-B/16+ at 69.2\%, and ViT-L/14 at 75.3\%)~\cite{Ilharco_OpenCLIP_2021}.
The difference between ResNet-50 and ResNet-101 within dataset YFCC15M is not significant, although there is a slight gap between these models in ImageNet zero-shot trends (32.7\% vs 34.8\%)~\cite{Ilharco_OpenCLIP_2021}.
Overall, we note that the LAION trained models (which are both larger models and trained on larger datasets) perform \textit{significantly} better than smaller models across both Tables \ref{tab:systematicity_weak_negs} and \ref{tab:systematicity_hard_negs}.

We observe similar trends in figure \ref{fig:prodModelPerf} (productivity), with ViT-L/14 models performing generally strongest across complexities, ViT-B/16+ outperforming ViT-B/16, and ViT-B/32 underperforming.
There is again no clear difference between ResNet-50 and ResNet-101 trained on YFCC15M.
Taken together, these results suggest that retrieval performance rankings are consistent with rankings of zero-shot ImageNet accuracy, with larger models (\eg ViT-L/14) generally outperforming smaller models (\eg ViT-B/16) within LAION-400M.

% \begin{figure*}[t]
%      \centering
%      \includegraphics[width=\linewidth]{figures/Complexity Figure.jpg}
%      \caption{A figure denoting how productivity experiment performance varies based on the complexity of the evaluated captions. Different lines represent different models. I only included R@1 and the negative of GT-HN1 (average of ground truth rank minus min. hard-negative type 1 rank). Other metrics should naturally also be included. If warranted, these figures could focus on particular templates rather than overall performance for a given complexity.}
%      \label{fig:ex5}
%  \end{figure*}

% \input{tables/productivity_overall}



==> old/05_experiments_v2.tex <==


\section{Experiments}
We detail our experimental setup and then present our results with six key takeaways. First, our systematicity experiments show performance decreases consistently on compounds unseen during training. Second, the greatest drop between splits occurs for models trained on the largest dataset. Third, our productivity results reveal models' abilities to retrieve ground-truth captions decay with increasing complexity. Fourth, we find that dataset size has no impact on this observation. Fifth, we find no clear trend relating model size to compositionality. Finally, we find that models' ranking on zero-shot ImageNet classification correlates with their rankings for compositionality.

\noindent\textbf{Datasets} 
For our experiments, we utilize Visual Genome to form our test datasets. For systematicity, the image patches and corresponding spelling-corrected region descriptions are used.
% ; parsing errors are reduced by the fact that descriptions already have ground truth annotated scene graphs associated with them. 
We produce a $\D_{test}^{RAW}$ and a $\D_{test}^{HN}$ dataset for three training datasets: CC-12M, YFCC-15M and LAION-400M. For productivity, Visual Genome's image-scene graph pairs are used to create captions and hard negatives for $\D_{test}^{RAW}$ and $\D_{test}^{HN}$. Refer to Table \ref{tab:dataset_summary} for a detailed breakdown.

% Note that for productivity, $\D_{test}^{HN}= \cup_{n, i} \D_{test}^{HN(n, i)}$, and 


\noindent\textbf{Models} We evaluate seven vision-language models pretrained with the CLIP loss~\cite{radford2021learning} across three commonly used image-text datasets: Conceptual Captions 12M (CC-12M)~\cite{changpinyo2021conceptual}, a subset of the YFCC100M dataset (YFCC-15M)~\cite{thomee2016yfcc100m, radford2021learning} and LAION-400M~\cite{schuhmann2021laion}. We limit our evaluation to models openly released in the OpenCLIP repository~\cite{Ilharco_OpenCLIP_2021}. 
These include ResNet (RN)~\cite{he2016deep} and Vision Transformer (ViT)~\cite{dosovitskiy2021an} encoders of different sizes: RN50, RN101, ViT-B-16, ViT-B-16-plus-240, ViT-B-32 and ViT-L-14.

\noindent\textbf{Metrics} For $\D^{HN}_{test}$, we adopt commonly used retrieval metrics Recall@1, 3, 5 and Average Recall@K. For $\D^{RAW}_{test}$, we report the mean and standard deviation of Recall@1 across K-fold retrievals (where $K = \min(20, \lfloor \frac{|\D^{RAW}_{test}|}{N} \rfloor)$, and $N = \min(|SC|, |UC|, |UA|) = 1855$), as the data size varies across compositional splits and complexities.
% where at each fold we \textit{resample from the set of feasible hard negatives for each ground truth caption for productivity and resample from the compositional split in systematicity.}

\input{figures/modelPerfvsRecall_syst.tex}
\subsection{Systematicity evaluation}
\paragraph{Model performance decreases monotonically when compounds are unseen.} This is the case for both $\D^{HN}_{test}$ (Table \ref{tab:systematicity_hard_negs}) and $\D^{RAW}_{test}$ (Table \ref{tab:systematicity_weak_negs}). 
This drop is consistently smaller ($2\%$ relative drop) for models trained on CC-12M and YFCC-15M, but pronounced ($5\%$ or higher, reaching $7.9\%$ drop for Vit-B-32) for LAION-400M models.
% For instance on $\D^{ret}_{HN}$, LAION-400M models, with the exception of ViT-L-14, experience Recall@1 drops of approximately $5\%$ or higher, with the relative drop in performance from Seen all compounds (SC) values reaching $16.29\%$ for Vit-B-32. 
However, CC-12M and YFCC-15M models also significantly underperform LAION-400M models in general, meaning that small drops between sets may be due to overall poor performance rather than improved systematic generalization. In comparison, human oracle experiments generalize with $100\%$ accuracy to $\D^{HN}_{test}$.

\noindent\textbf{Systematicity performance drop is more pronounced for larger training datasets.} 
We observe a clear gap in performance with stratifying across pretraining datasets, with LAION-400M models scoring much higher (Table~\ref{tab:systematicity_hard_negs}). This gap decreases as we relax the evaluation metric, with Recall@ 5 being close across models trained on all datasets on both seen and unseen compounds splits. 

% We also observe that the recall drop between the Seen Compounds and Unseen Compounds splits is \textit{steeper} for larger models trained on larger datasets; \ie while CC-12M models only drop 2 percentage points in R@1 between the two splits, LAION models drop up to 8 percentage points between the Seen and Unseen splits.

\input{figures/modelPerfvsRecall_prod.tex}
\input{figures/produtivity_hard_negs_plot}

When comparing these values in the original RAW dataset without hard negatives, (Table \ref{tab:systematicity_weak_negs}), we see a similar drop in performance for LAION-trained models across both the image-to-text and text-to-image tasks.
We also observe larger drops on LAION-trained models when moving across the $\textsc{SC}\to \textsc{UC}$, and across $\textsc{UC}\to \textsc{UA}$ splits, with LAION models dropping as much as $13\%$ for ViT-L/14.


\subsection{Productivity evaluation}
\paragraph{Models' performance decreases with complexity on $\textsc{HN-Atom}$ and $\textsc{HN-Swap}$ negatives.} 
At small complexities such as $n=4$, we observe that model retrieval  quality is well above random chance  (Figure \ref{fig:prod_hard_negs}). However, as caption complexity increases, we observe a steady decrease in performance, nearing random chance for $\textsc{HN-ATOM}$ and dipping below it for $\textsc{HN-SWAP}$ negatives. 
% While past work demonstrates that vision-language models struggle with atomic~\cite{parcalabescu-etal-2022-valse, park-etal-2022-exposing} and swapping~\cite{thrush2022winoground, yuksekgonul2022and} foils, 
Our results demonstrate that the challenge of differentiating between atomic and swapping foils is exacerbated by caption complexity. 
% For $\textsc{HN-NEG}$ foils, we do not observe a downward trend, as model performance is generally stable but poor.

\noindent\textbf{We see no effect of dataset size on productivity.} Unlike the systematicity experiments, we do not observe a clear advantage for larger pretraining datasets in this set of experiments.
For atomic and swapping foils, we see similar performance for models trained on the three datasets, with slightly worse performance on atomic foils for the model trained on CC-12M. 
% When the hard negative type is atomic foils (Figure \ref{fig:prod_hard_negs}, left), we see similar performance for models trained on LAION-400M and YFCC-15M, with slightly worse performance overall for the model trained on CC-12M. 
% When the hard negative type is swaps (Figure \ref{fig:prod_hard_negs}, right), we see that all models (across all datasets) show similar retrieval perofrmance.
However, when the hard negative type is negations (Figure \ref{fig:prod_hard_negs}, center), we see variable performance based on pretraining dataset, with CC-12M models (the smallest model and smallest dataset) outperforming LAION and YFCC models (larger models on larger datasets).

% We note that, in our results, there is no clear pattern suggesting that larger pretraining datasets (for which we also test larger models) lead to better retrieval performance.
% To isolate the influence of pretraining dataset from model architecture, we also compare group results on model type and compare across datasets in Figure \irena{I think Mona is working on this}.
% We see that \irena{todo once we have this analysis}.
% \irena{Discussion if the results are interesting.} We note that, in addition to differing in their sizes (12M, 15M, and 400M), these pretraining datasets also differ in their filtering protocol, with CC-12M particularly optimizing for entity coverage~\cite{changpinyo2021conceptual}. 

% \irena{
%     the tricky part here is that the model sizes are conflated with the pretraining dataset. we have 
%     CC-12M: RN50(23M), 
%     YFCC: RN50(23M), RN101 (44M),
%     LAION: ViT-B-16(86M), VitB16p(), VitB32(197M), Vitl14(307M)
% }

\subsection{Effect of model size}
\noindent\textbf{We find no trends relating compositionality to model size.}
Across both systematicity (Figure~\ref{fig:systModelPerf}) and productivity (Figure~\ref{fig:prodModelPerf}), model performance remains indifferent to the size of the model itself. 
% That being said, future work should re-run this experiment once more vision-language foundation models become publicly available. 
Overall, we note that the LAION trained models (which are both larger models and trained on larger datasets) perform \textit{significantly} better than smaller models across both Tables \ref{tab:systematicity_weak_negs} and \ref{tab:systematicity_hard_negs}.


% Lastly, we also compare retrieval ability across model sizes within a pretraining dataset (Figure \ref{fig:prodModelPerf}).
% We examine two datasets for this section: YFCC-15M (for which we evaluate a ResNet50 and a ResNet101) and LAION-400M (for which we evaluate ViT-B/16, Vit-B/16+, ViT-B/32, and ViT-L/14).

% In figure \ref{fig:systModelPerf} (systematicity) we observe that larger models tend to have better retrieval abilities within LAION-400M, for which we have four models to compare. 

\subsection{Correlation with ImageNet zero-shot}
\noindent\textbf{We find that zero-shot ImageNet performance correlates with compositionality.}
The relative rankings of models on systematicity as well as productivity is correlated with their ranking on zero-shot ImageNet accuracy as reported by the OpenCLIP authors (where ViT-B/32 performs worst at 62.9\%, than ViT-B/16 at 67.1\% and ViT-B/16+ at 69.2\%)~\cite{ilharco_gabriel_2021_5143773}.
% and ViT-L/14 at 75.3\%)~\cite{Ilharco_OpenCLIP_2021}.
We do not observe this correlation for ResNets within YFCC-15M.
% The difference between ResNet-50 and ResNet-101 within dataset YFCC-15M is small, although there is a difference between them in ImageNet zero-shot trends ($32.7\%$ vs $34.8\%$)~\cite{ilharco_gabriel_2021_5143773}.

%We observe similar trends in figure \ref{fig:prodModelPerf} (productivity), with ViT-L/14 models performing generally strongest across complexities, ViT-B/16+ outperforming ViT-B/16, and ViT-B/32 underperforming.
% There is again no clear difference between ResNet-50 and ResNet-101 trained on YFCC-15M.
% Taken together, these results suggest that retrieval performance rankings are consistent with rankings of zero-shot ImageNet accuracy, with larger models (\eg ViT-L/14) generally outperforming smaller models (\eg ViT-B/16) within LAION-400M.

% \begin{figure*}[t]
%      \centering
%      \includegraphics[width=\linewidth]{figures/Complexity Figure.jpg}
%      \caption{A figure denoting how productivity experiment performance varies based on the complexity of the evaluated captions. Different lines represent different models. I only included R@1 and the negative of GT-HN1 (average of ground truth rank minus min. hard-negative type 1 rank). Other metrics should naturally also be included. If warranted, these figures could focus on particular templates rather than overall performance for a given complexity.}
%      \label{fig:ex5}
%  \end{figure*}

% \input{tables/productivity_overall}



==> old/06_discussion_v1.tex <==

\section{Discussion}

\noindent\textbf{Limitations.} There are three key limitations associated with our evaluation. First, although our data validation protocols verified our generated hard negatives for productivity as high-quality, less than $78.1\%$ of \textsc{HN-Swap} and of \textsc{HN-Neg} negatives were rated as correct. While this does not invalidate our key productivity result, this noise is a limitation of \name{} and could hinder future evaluations once foundation models begin performing better. Second, given the computational requirements associated with training a foundation model, our experiments centered around model architectures that were already available publicly. We hope that future foundation models are evaluated with our publicly available \name{} benchmark. Third, while we observed text-to-image and image-to-text retrieval to have similar trends for our systematicity experiments, we lack text-to-image datasets with hard negatives. Future work can explore mechanisms to generate counterfactual negative images.

\noindent\textbf{Conclusion.}
We presented \nameemoji{}, a collection of text-to-image and image-to-text retrieval datasets for the evaluation of pretrained vision-language models' systematicity and productivity. We demonstrate that models are not compositional along both axes, with performance drops across different compositional splits and increasing complexity.
We expect that \name{} will provide a more systematic evaluation of future vision-language foundation models, allowing researchers to benchmark the emergence of compositionality as models improve.
Finally, our results indicate an opportunity where researchers can leverage our hard-negative generation process to create training batches with hard negatives to incentivize vision-language compositionality.

==> old/scratch.tex <==
Comparative psychology, specifically Morgan's Canon~\cite{morgan1894introduction}, has come to appreciate that human researchers are vulnerable to systematic biases when comparing human and nonhuman intelligence. Understood as an error, Morgan's Canon is the tendency of people to attribute human-like characteristics to non-humans on the basis of insufficient empirical evidence. In an effort to avoid this error in interpreting the emergent machine capabilities~\cite{buckner2019comparative}, this paper focuses on evaluating today's popular vision-language foundation models. Given our learned models' propensity for shortcut learning~\cite{geirhos2020shortcut}, wherein they maximize benchmark performance while failing to generalize to real applications, it is vital that we uncover deficiencies in model behavior. Understanding model behavior is particularly especially for foundation models, such as CLIP~\cite{radford2021learning}, which has ubiquitously become the ``foundation'' atop which other models are trained~\cite{conwell2022testing,ramesh2022hierarchical,saharia2022photorealistic}.


% paragraph about why measuring compositionality is hard.
Existing benchmarks used to evaluate vision-language models are insufficient for evaluating the emergence of compositional reasoning. These models are trained using web-scraped datasets, comprised of millions of images with their associated text captions~\cite{thomee2016yfcc100m,schuhmann2021laion,sharma2018conceptual}. The dominant training paradigm is a contrastive objective~\cite{radford2021learning}; the resulting model are evaluated using image-text retrieval over these large datasets~\cite{jia2021scaling,radford2021learning,Zhang_2021_CVPR}. Although these datasets contain rich compositional structure, we show that achieve a high performance on retrieval doesn't require compositionality. A test for compositional understanding requires images with captions containing similar words but different compositional rules (see Figure~\ref{fig:pull_figure}). Noticing this deficiency, important recent work has introduced a small test set with $400$ hand-crafted captions with word orders permuted~\cite{thrush2022winoground}. Although valuable, there is a need for larger benchmarks that test for a more ... \rak{need to say that we are different from winoground.}.

==> old/scratch_v2.tex <==
% New outline
    % State of the world
        % Option 1: 
            % Open with the importance of compositionality for human intelligence
            % Segue into pretrained vision-language models. Clumsy?
        % Option 2:
            % Open with the success and prevalence of pretrained vision-language models
            % 
    % What's missing
    % Why is it hard to fill up what's missing
    % Bit-flip
    % Our contribution
        % High-level idea
        % Specifics of the dataset with statistics
        % Insights and takeaways




==> old_tables/productivity_error_modes.tex <==

\begin{table*}[]
\centering
\label{tab:proderrors}
\begin{tabular}{l|p{0.45\textwidth}|p{0.45\textwidth}|l}
    $i$ & Error Mode  & Hard Negative & $h_i$ \\ \hline
    1   & As sentence complexity increases, the model may begin ignoring individual details.
    & \textbf{Atomic foils}. Replace one atom of the caption with a mutually exclusive atom.              & 8 \\ \hline
    2   & As sentence complexity increases, the model may begin acting like a bag of words, ignoring position, syntax, and proper binding. 
    & \textbf{Swapping foils}. Take two atoms of the same type within a caption and swap them. 
    & 8 \\ \hline
    3   & As sentence complexity increases, the model’s capacity to comprehend negations falter.
    & \textbf{Negation foils}. Negate an atom with a grammatically correct variant of “is not,'' or negate the entire caption. & 5
\end{tabular}
\caption{A list of the potential failure modes CLIP may encounter when parsing increasingly complex scenes, and the corresponding hard negatives generated in our retrieval sets to test CLIP accordingly. For a retrieval set $R_{n, i}$, $h_i$ is the number of hard negatives generated from each ground truth caption, all of which are retrieved against the corresponding image.}
\end{table*}


==> old_tables/productivity_overall.tex <==
\begin{table*}[]
\caption{A table denoting overall productivity performance, without splitting based on template complexity. After we refine templates, this table's rows could instead be based on template type. Performance based on foil type is captured implicitly by the rank difference metrics like GT-HN1.}
\label{tab:productivity_overall}
\centering
\begin{tabular}{lllll}
              & R@1 & GT-HN1 & GT-HN2 & GT-WN \\ \hline
CLIP (ResNet) &     &        &        &       \\
CLIP (ViT)    &     &        &        &       \\ \hline
\end{tabular}
\end{table*}

\begin{table}[]

\end{table}

==> old_tables/systematicity_by_split.tex <==
\begin{table*}[]
\caption{A table denoting systematicity performance on the main metrics (R@1, GT-HN1, GT-HN2, GT-WN) on each split (seen, novel, w/ unseen). For each split, we also report performance based on the template type. For the novel composition split, we also report performance based on what is novel. If we take note of relationship and attribute types, we can also have an appendix table further splitting over those.}
\label{tab:systematicity_split}
\centering
\begin{tabular}{llllllllll}
\multicolumn{2}{l}{\multirow{2}{*}{Split}}         & \multicolumn{4}{l}{CLIP (ResNet-50)} & \multicolumn{4}{l}{CLIP (ViT)} \\ \cline{3-10} 
\multicolumn{2}{l}{}                               & R@1   & GT-HN1   & GT-HN2   & GT-WN  & R@1  & GT-HN1 & GT-HN2 & GT-WN \\ \hline
\multirow{3}{*}{Seen}            & All             &       &          &          &        &      &        &        &       \\ \cline{2-2}
                                 & AO              &       &          &          &        &      &        &        &       \\ \cline{2-2}
                                 & SRO             &       &          &          &        &      &        &        &       \\ \cline{1-2}
\multirow{7}{*}{Novel}           & All             &       &          &          &        &      &        &        &       \\ \cline{2-2}
                                 & AO              &       &          &          &        &      &        &        &       \\ \cline{2-2}
                                 & SRO (all)       &       &          &          &        &      &        &        &       \\ \cline{2-2}
                                 & SRO (all novel) &       &          &          &        &      &        &        &       \\ \cline{2-2}
                                 & SRO (novel S)   &       &          &          &        &      &        &        &       \\ \cline{2-2}
                                 & SRO (novel R)   &       &          &          &        &      &        &        &       \\ \cline{2-2}
                                 & SRO (novel O)   &       &          &          &        &      &        &        &       \\ \cline{1-2}
\multirow{3}{*}{w/ Unseen Atoms} & All             &       &          &          &        &      &        &        &       \\ \cline{2-2}
                                 & AO              &       &          &          &        &      &        &        &       \\ \cline{2-2}
                                 & SRO             &       &          &          &        &      &        &        &       \\ \hline
\end{tabular}
\end{table*}


